Communication-Constrained Multi-Robot Exploration with Intermittent Rendezvous

Communication constraints can significantly impact robots' ability to share information, coordinate their movements, and synchronize their actions, thus limiting coordination in Multi-Robot Exploration (MRE) applications. In this work, we address these challenges by modeling the MRE application as a DEC-POMDP and designing a joint policy that follows a rendezvous plan. This policy allows robots to explore unknown environments while intermittently sharing maps opportunistically or at rendezvous locations without being constrained by joint path optimizations. To generate the rendezvous plan, robots represent the MRE task as an instance of the Job Shop Scheduling Problem (JSSP) and minimize JSSP metrics. They aim to reduce waiting times and increase connectivity, which correlates to the DEC-POMDP rewards and time to complete the task. Our simulation results suggest that our method is more efficient than using relays or maintaining intermittent communication with a base station, being a suitable approach for Multi-Robot Exploration. We developed a proof-of-concept using the Robot Operating System (ROS) that is available at: https://github.com/multirobotplayground/ROS-Noetic-Multi-robot-Sandbox.

==> DEPRECATED/5-method.tex <==
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{figures/outline.png}
\caption{Simplified general overview of the rendezvous integrated as a decouple action in a frontier-based method.}
\vspace{-2.0em}
\label{fig:outline}
\end{figure}

\section{Methodology}
\label{sec:method}

In our method, robots explore with an intermittent communication plan with a frontier-based exploration stack, as displayed in the Finite State Machine shown in Fig.~\ref{fig:outline}. During exploration, they can decide to follow an agreement with other robots generated in the \textit{generate plan} state. They follow a robust frontier-based method through the \textit{explore} and \textit{update frontiers} states. When they meet at specific locations to honor some agreements, through the \textit{go rendezvous} state. We update the team's entire intermittent communication plan and repeat the process when appropriate. Next, we introduce how we ensure intermittent communication.

Firstly, we propose creating a rendezvous plan as actions from $A_i$ that are dynamically updated as exploration happens with a frontier-based method. We define a rendezvous plan with two matrices, $\mathcal{W}$ and $\mathcal{K}$, and a tuple $l=(l_1,...,l_f)$ composed of rendezvous locations. Columns in both matrices represent robots, rows represent rendezvous agreements, and variables from $l$ are rendezvous locations assigned to each agreement. Each $w_{ij}$ from $\mathcal{W}$ is a binary variable, where robot $r_j$ should participate in the $i$th agreement if $w_{ij} = 1$. Differently, each $k_{ij}$ from $\mathcal{K}$ is a real value that specifies the number of exploration steps a robot should do before going to the $i$th rendezvous location in $l$.

\subsubsection{Agreement Fulfillment and Update}

Robots fulfill an agreement from the $i$th row of $\mathcal{W}$ when they meet at their assigned location from $l$. Agreements are fulfilled from the first to the last and repeat in order.
% If a robot participates in multiple agreements, it should try to fulfill them from the first to the last. Robots start over from their first assignment when they fulfill their last one. 
Every time robots fulfill their last agreement, we dynamically update all rendezvous locations inside $l$ and distribute new plans.
%\thales{is this corerct? after finishing the last agreement all rendezvous locations in l are updated?}. 
We purposefully let all robots participate in the last agreement from $\mathcal{W}$ and we define it as a synchronization point. We provide more insights about the synchronization later.

\subsubsection{Agreement Maintenance during Execution}
\label{sec:rendezvous_agreement}

During the exploration, we maintain agreements for a robot $r_j$ inside a circular list and keep track of the current one with a pointer that starts at its first element. Each element of this list is a tuple $(r_1^w,r_2^w,...,\mathcal{L}, \mathcal{Y}, id)$ of the $ith$ agreement from $\mathcal{W}$, where each $r_i^w$ is the unique identifier for a robot that $r_j$ should meet, $\mathcal{L}$ is a value ($k_{ij}$) from $\mathcal{K}$, $\mathcal{Y}$ is the rendezvous location ($l_i$) of this agreement, and $id$ is the $ith$ row number. We use the row number to identify the agreement the robots have to fulfill. We initialize all $\mathcal{Y}$ for all robots with the same starting position from $\Omega$. After $r_j$ fulfills its current agreement, we increment the pointer to the next one on the list and follow with subsequent exploration. A robot keeps track of how much time it is effectively exploring new locations, and if this time is higher than $\mathcal{L}$, it will navigate to its current agreement rendezvous location.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.35\textwidth]{figures/rendezvous_dynamic_update.png}
    \caption{Example of rendezvous locations $l_1$ to $l_4$ in Buckingham Palace, London, UK. The blue circles are frontiers used by the KNN algorithm and colored zones represent the areas that robots will prioritize.}
    \label{fig:dynamic_update}
    \vspace{-2.0em}
\end{figure}

\subsubsection{Dynamically Updating Rendezvous Locations}

We dynamically update the rendezvous locations from $l$ during execution for all agreements after all robots fulfill the synchronization point. 
We generate the new locations by running a modified K-Nearest Neighbors (KNN) algorithm to assemble a frontier set $F_c = \{f_{c1},f_{c2},...\}$, where $c$ stands for centroid, based on $\mathcal{F}_j$ given their nearest neighbors. Next, we select which $f_{ci}$ to assign as new rendezvous location. First, we pick the farthest $f_{ci}$ from the current synchronization location and add it to a control list. We do all the subsequent selections by picking a new frontier from $F_c$ with the maximum distance to all others already inserted into the control list. We repeat the process until we have picked enough frontiers to update all rendezvous locations inside $l$. Fig.~\ref{fig:dynamic_update} illustrates an example of new rendezvous locations for four agreements in one of our simulated environments. Finally, we update all $\mathcal{Y}$ variables from each circular list held by the robots. 
% \thales{Is this centralized?}

\subsection{Generating Rendezvous Agreements}

The rendezvous plan should enable robots to connect during the exploration. However, due to differences in values from matrix $\mathcal{K}$, robots can be locked, waiting for others more often, increasing the exploration time. To make plans repeatable, we generate them in three parts. The first is the agreement, which specifies how robots should communicate over time. Differently, the second one is a \textit{reduce}, making subgroups of robots meet and share maps to prepare for a full team meetup. The last part is an agreement between all robots we use to synchronize the plan, allowing a re-planing window. We propose to run an optimization procedure over a condensed proximity graph $\mathcal{G}_c$ and an instance $\mathcal{I}$ of the Job Shop Scheduling Problem (JSSP) \cite{Gao2019} obtained from a reduction on a rendezvous plan. Next, we propose the following reduction.

\begin{figure}[t!]
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_prefix_plan.png}
        \caption{Agreement}
        \label{fig:prefix_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_with_suffix_plan.png}
        \caption{Reduce}
        \label{fig:suffix_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_with_synchronizer_plan.png}
        \caption{Synchronize}
        \label{fig:synchronize_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/11_plans_example.png}
        \caption{Optimized}
        \label{fig:complex_example}
    \end{subfigure}
    \caption{Jobs with the same color allocated to different robots (lines) represent one rendezvous agreement. Robots should explore the environment until their job ends and go to the assigned rendezvous location. The X-axis represents time steps.}
    \label{fig:jssp_instances}
    \vspace{-1.5em}
\end{figure}

Before introducing our reduction algorithm, consider that machines in the JSSP instance are robots that can execute jobs. Also, consider that jobs are composed of tasks that robots should do, such as navigating and exploring a region through actions in $\mathcal{A}_i$.

\subsubsection{Reduction to JSSP Instance}

Let $\mathcal{I}$ be an instance of a JSSP containing $|\mathcal{R}|$ machines that represent the rendezvous plan agreements for a sequence of time steps. Consider that $\mathcal{W}$ and $\mathcal{K}$ were given and that the execution time of a job is the total time needed to trigger a plan obtained from $\mathcal{K}$. Furthermore, consider that jobs have an identifier to show which row of $\mathcal{W}$ they are associated. We store an array $t_{\mathcal{I}}$ that holds the ending time of the previously allocated jobs for all machines and use it to create new jobs. Next, for each row $i$ of $\mathcal{W}$, we verify which robots should participate in the agreement and create a new job $j$ with length $k_{ij}$ for each. We set the starting time of each newly-created $j$ as $\max(t)$ for all participating robots to ensure locking resources, set ending time as $t_i + k_{ij}$, and set their identifier to $i$. We store the ending times of the current iteration inside a list $t_e$. Finally, we update $t_i$ from the participating robots as $\max(t_e)$, store all jobs in a jobs list $J_{\mathcal{I}}$ and repeat the process until all agreements are processed. 

From the JSSP instance $\mathcal{I}$, we calculate the normalized total number of jobs as

\begin{equation}
\label{eq:num_plans}
g_1(\mathcal{I}) = |J_{\mathcal{I}}|\mu_1
\end{equation}

\noindent
where $\mu_1$ is a normalization factor; the total normalized exploration steps 

\begin{equation}
\label{eq:workdone}
g_2(\mathcal{I}) = (1+\sum_{\text{job}_i \in J_{\mathcal{I}}}{job}_i)^{-1}
\end{equation}

%\begin{equation}
%\label{eq:workdone}
%g_2(\mathcal{I}) = (1+\sum_{\text{job}_i \in J_{\mathcal{I}}}{job}_i\mathbb{E}(u_j))^{-1}
%\end{equation}

\noindent
where $\text{job}_i$ is the length of the $ith$ job from the jobs list $J_{\mathcal{I}}$; 
%and $\mathbb{E}(u_j)$ is the expected reward of robot $r_j$ that executes $job_i$; 
the normalized makespan

\begin{equation}
\label{eq:makespan}
g_3(\mathcal{I}) = max_{\forall t_i \in t_{\mathcal{I}}}(t_i)(1 + max_{\forall t_i \in t_{\mathcal{I}}}(t_i))^{-1}
\end{equation}

\noindent
where $t_{\mathcal{I}}$ is the ending times array we create during the reduction; and the normalized standard deviation of the distances between each agreement fulfillment

\begin{equation}
\label{eq:sigma_agreement}
g_4(\mathcal{I}) = \sigma_{\mathcal{I}}(1 + \sigma_{\mathcal{I}})^{-1}
\end{equation}

The intuition behind equations \ref{eq:num_plans} and \ref{eq:makespan} is to quantify how often robots share maps through the number of agreements per time step. We use eq.~\ref{eq:workdone} to measure how much exploration we expect to have and how much time they should explore before fulfilling their agreements through eq.~\ref{eq:sigma_agreement}. We exemplify the result of this reduction in Fig.~\ref{fig:prefix_jobs} for a plan composed of four robots and three agreements. We define plan locks as situations where robots wait for others at a rendezvous location. We illustrate these locks as white gaps in the JSSP instance from Fig.~\ref{fig:suffix_jobs}.

\subsubsection{Reduce Agreements}

Repeating the JSSP instance $\mathcal{I}$ will generate several locks because of the allocation shifts. Consequently, we generate a reduce structure to make the plan repeatable. We let the reduce be composed of $\lfloor \frac{n}{2} \rfloor$ new agreements if $n > 3$, where $n$ is the number of robots. Otherwise, we create only one new agreement. To assign robots to the created agreements, we put them into a queue and do the assignment while the queue has elements. At each iteration, we process two robots, $r_i$ and $r_j$, by removing them from the queue and creating new jobs, $j_i$ and $j_j$, with the same unique job identifier. We set the starting time of $j_i$ and $j_j$ as $t_i$ and $t_j$. Differently, we set their ending times as $t_i + \frac{\mu_{jobs}}{2}$ and $t_j + \frac{\mu_{jobs}}{2}$, respectively, where $\mu_{jobs}$ is the average job length. We update each element from $t$ with the newly created jobs ending time. In Fig.~\ref{fig:suffix_jobs}, we show the procedure results for four robots when appended into the JSSP instance $\mathcal{I}$ from Fig.~\ref{fig:prefix_jobs}. The intuition behind these new agreements is to make the rendezvous plan repeatable without adding extra locks.

\subsubsection{Synchronize Agreement}

To create a re-planning window where robots can dynamically update the entire rendezvous plan without adding locks, shifts, or undesired behaviors, we propose the concept of a synchronization agreement. Consequently, we create a new job for each robot, set their starting time to $t_i$ and ending time to $t_i + \frac{\mu_{jobs}}{2}$, and give them the same unique job identifier. We finally append all created jobs to $I$ as exemplified in Fig.~\ref{fig:synchronize_jobs}.

\subsubsection{Optimizing the Rendezvous Plan}

Let $\mathcal{H}$ be a function that generate a condensed proximity graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ that represents each time step in the JSSP instance $\mathcal{I}$. Robots use $\mathcal{G}$ to help evaluate the quality of the rendezvous plan. In this graph, an edge exists between two robots only if they have a common agreement from $\mathcal{I}$. From $\mathcal{G}$ a robot can extract the connectivity index

\begin{equation}
\label{eq:connectivity_index}
g_5(\mathcal{I}) =  \mathcal{C}(\mathcal{H}(\mathcal{I}))(1 + \mathcal{C}(\mathcal{H}(\mathcal{I})))^{-1}
\end{equation}

\noindent
where $\mathcal{C}(\mathcal{H}(\mathcal{I}))$ is a function that returns the length of the biggest connected component of $\mathcal{H}(\mathcal{I})$. A robot can also extract the number of edges

\begin{equation}
\label{eq:edges_count}
g_6(\mathcal{I}) = |\mathcal{E}_{\mathcal{H}(\mathcal{I})}|
\end{equation}

\noindent
where $\mathcal{E}_{\mathcal{H}(\mathcal{I})}$ is the set of edges from $\mathcal{G}$. The intuition behind eq.~\ref{eq:connectivity_index} is to check if the plan makes the robots intermittently share their maps. We use eq.~\ref{eq:edges_count} to count how many robots are inside the same agreement and try to distribute them accordingly.

To generate plans, we developed a customized SGA (Simple Genetic Algorithm) \cite{Tang1996} with genetic operators that allow us to iterate over solutions with different numbers of agreements and robots. Each individuals in the population holds a matrix $\mathcal{W}$ and $\mathcal{K}$. To evaluate them, we perform our JSSP reduction, create its condensed proximity graph, and minimize the following multi-objective optimization composed from equations \ref{eq:num_plans} to \ref{eq:edges_count}

\begin{align}
    \begin{split}
     I^* =& \ \underset{\mathcal{I}}{\arg\min} \ (g_1(\mathcal{I}),... , g_5(\mathcal{H}(\mathcal{I})), g_6(\mathcal{H}(\mathcal{I}))) \\
        & \quad \text{s.t.} \\
        & g_1(\mathcal{I}), ..., g_6(\mathcal{H}(\mathcal{I})) \geq 0
    \end{split}
\end{align}

\noindent
where the intuition behind this optimization is to generate a plan where the robots will keep exploring as much as possible at the cost of sharing their maps.

==> DEPRECATED/JSSP.tex <==
\subsection{Generating Rendezvous Agreements}

The rendezvous plan should enable robots to connect during the exploration. However, due to differences in values from matrix $\mathcal{K}$, robots can be locked, waiting for others more often, increasing the exploration time. To make plans repeatable, we generate them in three parts. The first is the agreement, which specifies how robots should communicate over time. Differently, the second one is a \textit{reduce}, making subgroups of robots meet and share maps to prepare for a full team meetup. The last part is an agreement between all robots we use to synchronize the plan, allowing a re-planing window. We propose to run an optimization procedure over a condensed proximity graph $\mathcal{G}_c$ and an instance $\mathcal{I}$ of the Job Shop Scheduling Problem (JSSP) \cite{Gao2019} obtained from a reduction on a rendezvous plan. Next, we propose the following reduction.

\begin{figure}[t!]
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_prefix_plan.png}
        \caption{Agreement}
        \label{fig:prefix_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_with_suffix_plan.png}
        \caption{Reduce}
        \label{fig:suffix_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/4_robots_with_synchronizer_plan.png}
        \caption{Synchronize}
        \label{fig:synchronize_jobs}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.24\columnwidth}
        \includegraphics[width=\linewidth]{figures/11_plans_example.png}
        \caption{Optimized}
        \label{fig:complex_example}
    \end{subfigure}
    \caption{Jobs with the same color allocated to different robots (lines) represent one rendezvous agreement. Robots should explore the environment until their job ends and go to the assigned rendezvous location. The X-axis represents time steps.}
    \label{fig:jssp_instances}
    \vspace{-1.5em}
\end{figure}

Before introducing our reduction algorithm, consider that machines in the JSSP instance are robots that can execute jobs. Also, consider that jobs are composed of tasks that robots should do, such as navigating and exploring a region through actions in $\mathcal{A}_i$.

\subsubsection{Reduction to JSSP Instance}

Let $\mathcal{I}$ be an instance of a JSSP containing $|\mathcal{R}|$ machines that represent the rendezvous plan agreements for a sequence of time steps. Consider that $\mathcal{W}$ and $\mathcal{K}$ were given and that the execution time of a job is the total time needed to trigger a plan obtained from $\mathcal{K}$. Furthermore, consider that jobs have an identifier to show which row of $\mathcal{W}$ they are associated. We store an array $t_{\mathcal{I}}$ that holds the ending time of the previously allocated jobs for all machines and use it to create new jobs. Next, for each row $i$ of $\mathcal{W}$, we verify which robots should participate in the agreement and create a new job $j$ with length $k_{ij}$ for each. We set the starting time of each newly-created $j$ as $\max(t)$ for all participating robots to ensure locking resources, set ending time as $t_i + k_{ij}$, and set their identifier to $i$. We store the ending times of the current iteration inside a list $t_e$. Finally, we update $t_i$ from the participating robots as $\max(t_e)$, store all jobs in a jobs list $J_{\mathcal{I}}$ and repeat the process until all agreements are processed. 

From the JSSP instance $\mathcal{I}$, we calculate the normalized total number of jobs as

\begin{equation}
\label{eq:num_plans}
g_1(\mathcal{I}) = |J_{\mathcal{I}}|\mu_1
\end{equation}

\noindent
where $\mu_1$ is a normalization factor; the total normalized exploration steps 

\begin{equation}
\label{eq:workdone}
g_2(\mathcal{I}) = (1+\sum_{\text{job}_i \in J_{\mathcal{I}}}{job}_i)^{-1}
\end{equation}

%\begin{equation}
%\label{eq:workdone}
%g_2(\mathcal{I}) = (1+\sum_{\text{job}_i \in J_{\mathcal{I}}}{job}_i\mathbb{E}(u_j))^{-1}
%\end{equation}

\noindent
where $\text{job}_i$ is the length of the $ith$ job from the jobs list $J_{\mathcal{I}}$; 
%and $\mathbb{E}(u_j)$ is the expected reward of robot $r_j$ that executes $job_i$; 
the normalized makespan

\begin{equation}
\label{eq:makespan}
g_3(\mathcal{I}) = max_{\forall t_i \in t_{\mathcal{I}}}(t_i)(1 + max_{\forall t_i \in t_{\mathcal{I}}}(t_i))^{-1}
\end{equation}

\noindent
where $t_{\mathcal{I}}$ is the ending times array we create during the reduction; and the normalized standard deviation of the distances between each agreement fulfillment

\begin{equation}
\label{eq:sigma_agreement}
g_4(\mathcal{I}) = \sigma_{\mathcal{I}}(1 + \sigma_{\mathcal{I}})^{-1}
\end{equation}

The intuition behind equations \ref{eq:num_plans} and \ref{eq:makespan} is to quantify how often robots share maps through the number of agreements per time step. We use eq.~\ref{eq:workdone} to measure how much exploration we expect to have and how much time they should explore before fulfilling their agreements through eq.~\ref{eq:sigma_agreement}. We exemplify the result of this reduction in Fig.~\ref{fig:prefix_jobs} for a plan composed of four robots and three agreements. We define plan locks as situations where robots wait for others at a rendezvous location. We illustrate these locks as white gaps in the JSSP instance from Fig.~\ref{fig:suffix_jobs}.

\subsubsection{Reduce Agreements}

Repeating the JSSP instance $\mathcal{I}$ will generate several locks because of the allocation shifts. Consequently, we generate a reduce structure to make the plan repeatable. We let the reduce be composed of $\lfloor \frac{n}{2} \rfloor$ new agreements if $n > 3$, where $n$ is the number of robots. Otherwise, we create only one new agreement. To assign robots to the created agreements, we put them into a queue and do the assignment while the queue has elements. At each iteration, we process two robots, $r_i$ and $r_j$, by removing them from the queue and creating new jobs, $j_i$ and $j_j$, with the same unique job identifier. We set the starting time of $j_i$ and $j_j$ as $t_i$ and $t_j$. Differently, we set their ending times as $t_i + \frac{\mu_{jobs}}{2}$ and $t_j + \frac{\mu_{jobs}}{2}$, respectively, where $\mu_{jobs}$ is the average job length. We update each element from $t$ with the newly created jobs ending time. In Fig.~\ref{fig:suffix_jobs}, we show the procedure results for four robots when appended into the JSSP instance $\mathcal{I}$ from Fig.~\ref{fig:prefix_jobs}. The intuition behind these new agreements is to make the rendezvous plan repeatable without adding extra locks.

\subsubsection{Synchronize Agreement}

To create a re-planning window where robots can dynamically update the entire rendezvous plan without adding locks, shifts, or undesired behaviors, we propose the concept of a synchronization agreement. Consequently, we create a new job for each robot, set their starting time to $t_i$ and ending time to $t_i + \frac{\mu_{jobs}}{2}$, and give them the same unique job identifier. We finally append all created jobs to $I$ as exemplified in Fig.~\ref{fig:synchronize_jobs}.

\subsubsection{Optimizing the Rendezvous Plan}

Let $\mathcal{H}$ be a function that generate a condensed proximity graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ that represents each time step in our JSSP instance $\mathcal{I}$. We use $\mathcal{G}$ to help evaluate the quality of the rendezvous plan. We create an edge between two robots only if they have a common agreement from $\mathcal{I}$ that can be fulfilled. From $\mathcal{G}$ we extract the connectivity index

\begin{equation}
\label{eq:connectivity_index}
g_5(\mathcal{I}) =  \mathcal{C}(\mathcal{H}(\mathcal{I}))(1 + \mathcal{C}(\mathcal{H}(\mathcal{I})))^{-1}
\end{equation}

\noindent
where $\mathcal{C}(\mathcal{H}(\mathcal{I}))$ is a function that returns the length of the biggest connected component of $\mathcal{H}(\mathcal{I})$. We also extract the number of edges

\begin{equation}
\label{eq:edges_count}
g_6(\mathcal{I}) = |\mathcal{E}_{\mathcal{H}(\mathcal{I})}|
\end{equation}

\noindent
where $\mathcal{E}_{\mathcal{H}(\mathcal{I})}$ is the set of edges from $\mathcal{G}$. The intuition behind eq.~\ref{eq:connectivity_index} is to see if the plan makes the robots intermittently share their maps if repeated. We use eq.~\ref{eq:edges_count} to count how many robots are inside the same agreement.

To generate plans, we developed a customized SGA (Simple Genetic Algorithm) \cite{Tang1996} with genetic operators that allow us to iterate over solutions with different numbers of agreements and robots. Each individuals in the population holds a matrix $\mathcal{W}$ and $\mathcal{K}$. To evaluate them, we perform our JSSP reduction, create its condensed proximity graph, and minimize the following multi-objective optimization composed from equations \ref{eq:num_plans} to \ref{eq:edges_count}

\begin{align}
    \begin{split}
     I^* =& \ \underset{\mathcal{I}}{\arg\min} \ (g_1(\mathcal{I}),... , g_5(\mathcal{H}(\mathcal{I})), g_6(\mathcal{H}(\mathcal{I}))) \\
        & \quad \text{s.t.} \\
        & g_1(\mathcal{I}), ..., g_6(\mathcal{H}(\mathcal{I})) \geq 0
    \end{split}
\end{align}

\noindent
where the intuition behind this optimization is to generate a plan where the robots will keep exploring as much as possible at the cost of sharing their maps at a rate. We provide an example of a JSSP instance for a plan we generate with our method in Fig.~\ref{fig:complex_example}.

==> DEPRECATED/algorithms/exploration.tex <==
\subsection{Multi-robot Frontier Exploration with Prioritization}

To perform exploration in line $18$ of Algorithm~\ref{alg:smainloop}, robots use the concept of frontiers, which are the boundaries of what is know and unknown. 
%
To select which frontier to explore, robots use an utility function $u(f_i)$ described in eq.~\ref{eq:frontier_utility}, where $\mathcal{N}_{f_i}$ is the amount of area uncovered by the robot and $\phi(f_i)$ is the path cost if visiting the frontier $f_i$.
%
In our exploration utility function, robots also use the concept o prioritization proposed by \cite{Solanas2004}, where they decide where to explore based on a positive or negative weight in the utility function. 
%
In our case, we let the robots explore regions that are in the direction of their next meet-up location so they can be closer to them when attending an agreement.
%
To check if they are going to explore the right place, we use the inner product $\langle\Vec{xf_i}, \Vec{yf_i} \rangle$, where $x$ is the center of mass of the local map and $y$ is the next meetup location. 
%
Even in the case of two robots exploring the same area due to the lack of proper communication, the reward function can be approximated by a discrete sum of the utility function for each robot.

\begin{equation}
\label{eq:frontier_utility}
u(f_i) = \alpha \frac{\mathcal{N}_{f_i}}{\Phi(f_i)} + \beta \langle\Vec{xf_i}, \Vec{yf_i} \rangle
\end{equation}

In Algorithm~\ref{alg:robotAlloc} we describe the procedures that robots use with the utility function for the single and multi-robot cases that are in accordance with the frontier-exploration literature \cite{yamauchi1999, Solanas2004, Burgard2005, Spirin2014, Caccavale2019, Bramblett2022, Soni2022, Tang2022}.
%
The algorithm works around the variable $\mathcal{F}_{choice}$, where it holds which frontier each nearby robot should select to maximize their $u_i(f_i)$. We expressed the selection as an iterative sampling process due to the size of the search space. However, for fewer robots the computation can be done efficiently in a single pass.

\subsubsection{\textbf{Single Robot Case}}

If a robot can not communicate, then $\mathcal{F}_{choice}$ should have only the selection (i.e., the frontier this robot selected) and the equation in line $13$ will turn into $u(f_i)$.

\subsubsection{\textbf{Multi-robot Case with Opportunistic Interactions}}

Otherwise, if a robot can communicate with other robots, then $\mathcal{F}_{choice}$ will contain the decisions each nearby robot should do to maximize a \textit{Social Welfare} function $\sum_{\forall f_i \in \mathcal{F}_{choice}} u_i(f_i)$.
%
This situation is expressed in the conditional in line $4$, which provides opportunistic coordination. 

The objective of the Social Welfare is to make robots do a joint-selection of frontiers to explore that maximizes the utility of the sub-team that can communicate in a given time step.
%
In line $11$ they apply a penalization if two robots select the same place to explore and in line $14$ they check if the current selection $\mathcal{F}_{choice}$ is better than the previous one due to the iterative process.

\subsubsection{\textbf{Distributed Computation}}

The computation of the $SW(\mathcal{F}_{choice})$ is done in a distributed fashion, because it is likely that robots within communication range will have the same map.
%
To accomplish the distributed computation, each robot should have access to the relative pose of its nearby neighbors to correctly estimate $u_i(f_i)$.

\begin{algorithm}
\DontPrintSemicolon
\KwIn{Frontier set $\mathcal{F}$}
\SetKwBlock{Begin}{function}{end function}
\SetKwRepeat{Do}{do}{while}
\Begin($\text{Exploration} {(\mathcal{F})}$) {
    \If{have a frontier $f$ to explore} {
        Try to navigate towards the frontier $f$\;
    } \uElseIf{found another robot when navigating \textbf{or} \\ \quad\quad\quad have not selected a frontier $f$ to explore \textbf{or} \\
    \quad\quad\quad finished navigation} {
            Let $\mathcal{F}_{best}$ to hold the best selection of frontiers so far for all nearby robots and initialize it to an empty set;\;
            \Do{stopping criteria} {
                Let $\mathcal{F}_{choice}$ be a hypothetical selection of frontiers to explore from $\mathcal{F}$ of each robot that I can communicate with, myself included, one time-step into the future;\;
                Let $f_i \in \mathcal{F}$ be the selected frontier from robot $i$;\;
                \If{two robots $i$ and $j$ select the same place to explore from $\mathcal{F}$} {
                    $u_i(f_i) = -u_i(f_i)$ and $u_j(f_j) = -u_j(f_j)$;\;
                }
                Let the \textit{Social Welfare} $SW(\mathcal{F})$ be $\sum_{\forall f_i \in \mathcal{F}_{choice}} u_i(f_i)$;\;
                \If{$SW(\mathcal{F}_{choice}) > SW(\mathcal{F}_{best})$} {
                    Update the best choice so far $\mathcal{F}_{best} \leftarrow \mathcal{F}_{choice}$;\;
                }
             }
            Set $f$ as the frontier this robot selected to explore from the choice $\mathcal{F}_{best}$;\;
    }
}
\caption{Multi-Robot Frontier Allocation}
\label{alg:robotAlloc}
\end{algorithm}

==> DEPRECATED/algorithms/frontier_old.tex <==
\section{Multi-robot Exploration with Intermittent Rendezvous}
\label{sec:explore}

In Algorithm~\ref{alg:smainloop}, we show how robots explore the environment and perform updates into the plan and sub-team rendezvous locations.
%
During each time step, a robot uses the Policy Components from fig.~\ref{fig:execution} to receive, share and merge maps, detect frontiers, and to navigate.
%
These components are used through lines $5$ to $8$ of the algorithm.
%
Differently, lines $11$-$19$ are responsible to fulfill the agreements, update sub-team locations, and update the plan.
%
In particular, $A_{cur}$ is a reference to the agreement from $K$ - that should be fulfilled next - and $steps$ is a reference to the number of explorations steps from $W$.
%
Importantly, a robot keeps local copies of $K$, $W$, and the merged map.

\begin{algorithm}
\small
\DontPrintSemicolon
\KwIn{Agreement matrix $K$\\
    \quad\quad\quad Exploration steps matrix $W$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{RendezvousFrontierExploration} {(K, W)}$) {
    Let $A_{cur}$ be the first agreement to fulfill $K$;\;
    Let $steps$ be the number of steps to explore from $W$;\;
    \ForEach{time step} {
        Receive maps from robots within communication range, merge with my map, and detect frontiers in the merged map;\;
        \If{there are no more frontiers to explore} {
            \textbf{break};\;
        }
        
        Select a frontier by optimizing a social function in a distributed fashion for robots within communication range;\;

        \If{exploring} {
            $steps = steps - 1$
        }
        \If{$steps \leq 0$} {
            meet the sub-team from $A_{cur}$ at its assigned location;\;
            \If{meeting occurred \textbf{and} \\
                \quad I am in charge of the update} {
                update the sub-team's rendezvous location while the others wait;\;
                \If{can update the plan} {
                    generate and distribute a new rendezvous plan $K$ and $W$;\;
                 }
            }\ElseIf{meeting occurred or timeout} {
                Set $A_{cur}$ to the next agreement this robot participates in $K$;\;
                Use $A_{cur}$ and $W$ to update $steps$;\;
            }
        }
    }
    Go back to the initial location;\;
}
\caption{Frontier Exploration with Rendezvous}
\label{alg:smainloop}
\end{algorithm}

\subsection{Frontier Utility}

A robot maximizes the following utility function when selecting frontiers to explore,

\begin{equation}
\label{eq:frontier_utility}
u(f_i) = \alpha \frac{\mathcal{N}_{f_i}}{\Phi(f_i)} + \beta \langle xf_i, yf_i \rangle
\end{equation}

\noindent
where, $\mathcal{N}_f$ is the amount of area that will be uncovered by visiting the frontier and $\Phi(f_i)$ is the cost of navigating towards $f_i$. 
%
The prioritization term $\langle xf_i, yf_i\rangle$ was originally proposed by \cite{Solanas2004} to assign robots to different exploration zones.
%
We modified it to represent the inner product between the vectors $xf_i = (f_i - x)$ and $yf_i = (f_i - y)$, where $x$ is the local map center of mass and $y$ is the current rendezvous location.
%
If $yf_i$ is headed to the place where robot should meet, then $\langle xf_i, yf_i\rangle$ yields a positive value.

\subsubsection{Selecting Frontiers with a Social Function}

At line $8$ of Algorithm~\ref{alg:smainloop}, a robot selects and explores frontiers for the single and multi-robot cases.
%
To select frontiers, let the variable $\mathcal{F}_{choice} = \{f_s,...,f_e\}$ be a hypothetical choice, where each $f_i \in \mathcal{F}_{choice}$ implies that robot $i$ selected $f_i$ to explore.
%
The objective of line $8$ is to find 

\begin{equation*}
\mathcal{F}^*_{choice} = \argmaxnew_{\mathcal{F}_{choice}} \sum_{f_i} u_i(f_i)
\end{equation*}

\noindent
for each robot $i$ within communication range, where $u_i(f_i)$ is the utility function from eq.~\ref{eq:frontier_utility} for robot $i$.
%
We call this summation as a social function, because its objective is to provide a distributed selection mechanism that maximizes the utility of the sub-team within communication range.
%
A robot explores the selected frontier from the outcome until it is possible.

The single and multi-robot cases work as follows:

% We call this summation as a social function, since it is distributed with the common goal of making each robot select a frontier that maximizing the sub-team utility.
% %
% To perform this computation in a distributed fashion, we let each robot of the sub-team known the relative pose of the others.

% We described the frontier selection as an iterative sampling process from lines $8$-$15$ due to the size of the search space.
% %
% However, for fewer robots the computation can be done efficiently in a single pass.
% %
% Nevertheless, the algorithm can be replaced by any coordination method, such as the Sywap \cite{Bautin2013}.

\begin{itemize}

\item{\textbf{Single Robot:}} If a robot can not communicate with others, then $\mathcal{F}_{choice}$ should have only one element (i.e., the frontier a robot $i$ selected) and the social function will turn into $u(f_i)$.

\item{\textbf{Multi-robot:}} Otherwise, if a sub-team is within communication range, each robot will calculate its own $\mathcal{F}^*_{choice}$ to select their frontiers.
%
If robots within communication range have equivalent merged maps, then they are going to achieve the same outcome.
%
To calculate the path cost of each $u_i(f_i)$, robots within communication range share their relative poses through the components from fig.~\ref{fig:execution}.
% 
% To mitigate the changes of exploring the same place, the algorithm applies a penalization into the social function if two frontiers from $\mathcal{F}_{choice}$, $f_i$ and $f_j$, are the same.
% %
\end{itemize}

For a smaller team of robots, it is possible to iterate over all possible outcomes of $\mathcal{F}_{choice}$ in the multi-robot case.
%
Differently, one should consider using Random Sampling to obtain an approximation or using a Multi-robot Wavefront propagation method instead (e.g., Sywap \cite{Bautin2013}) for a larger number of robots.

% \subsubsection{\textbf{Distributed Computation}}

% The computation of the $SW(\mathcal{F}_{choice})$ is done in a distributed fashion, because it is likely that robots within communication range will have the same map.
% %
% To accomplish the distributed computation, each robot should have access to the relative pose of its nearby neighbors to correctly estimate $u_i(f_i)$.

% \begin{algorithm}
% \DontPrintSemicolon
% \KwIn{Frontier set $\mathcal{F}$}
% \SetKwBlock{Begin}{function}{end function}
% \SetKwRepeat{Do}{do}{while}
% \Begin($\text{Exploration} {(\mathcal{F})}$) {
%     \If{have a frontier $f$ to explore} {
%         Try to navigate towards the frontier $f$\;
%     } \uElseIf{found another robot when navigating \textbf{or} \\ \quad\quad\quad have not selected a frontier $f$ to explore \textbf{or} \\
%     \quad\quad\quad finished navigation} {
%             Let $\mathcal{F}_{best}$ to hold the best selection of frontiers so far for all nearby robots and initialize it to an empty set;\;
%             \Do{stopping criteria} {
%                 Let $\mathcal{F}_{choice}$ be a hypothetical selection of frontiers to explore from $\mathcal{F}$ of each robot within communication range one time-step into the future;\;
%                 Let $f_i \in \mathcal{F}$ be the selected frontier from robot $i$;\;
%                 \If{two robots $i$ and $j$ select the same place to explore from $\mathcal{F}$} {
%                     $u_i(f_i) = -u_i(f_i)$ and $u_j(f_j) = -u_j(f_j)$;\;
%                 }
%                 Let the \textit{Social Welfare} $SW(\mathcal{F})$ be $\sum_{\forall f_i \in \mathcal{F}_{choice}} u_i(f_i)$;\;
%                 \If{$SW(\mathcal{F}_{choice}) > SW(\mathcal{F}_{best})$} {
%                     Update the best choice so far $\mathcal{F}_{best} \leftarrow \mathcal{F}_{choice}$;\;
%                 }
%              }
%             Set $f$ as the frontier this robot selected to explore from the choice $\mathcal{F}_{best}$;\;
%     }
% }
% \caption{Multi-Robot Frontier Allocation}
% \label{alg:robotAlloc}
% \end{algorithm}

\subsection{Updating the Rendezvous Locations and Plan}

If a sub-team is attending an agreement, at line $12$ of Algorithm~\ref{alg:smainloop}, we let one of the robots from the sub-team compute a new meeting location and distribute it to the others. 
%
To calculate the new location, we propose to generate a set of centroids from all the available frontiers in the merged map and clustering them with a KNN (K-Nearest Neighbor Algorithm).
%
The robot performing the calculations samples one of the positions obtained from the KNN and distributes it among all the other robots from the sub-team.

When fulfilling a synchronization agreement, robots fall at the conditional at line $15$, which tells to update the plan with the synchronization method.
%
In this case, one robot from the agreement receives information from the team, generates a new plan, and distributes the new plan to the others.
%
After receiving the new location or plan, robots select the next agreement they should fulfill and continue exploring until there are no more frontiers left.

% \subsubsection{Agreement Maintenance}

% During the exploration, lines $14$ - $18$ of Algorithm~\ref{alg:smainloop}, robots perform multi-robot exploration by creating a map, merging maps from nearby robots, and selecting frontiers to explore based on which robots are nearby.
% %
% We explain this exploration process in Algorithm~\ref{alg:robotAlloc}.
% %
% Differently, line $19$ get the available resources from the current agreement and check if they were spent exploring new areas in the environment.
% %
% If a robot spent the resources needed to attend to the current agreement's location $l$, it will navigate towards it and wait for the sub-team to arrive.
% %
% When every robot of the sub-team is at the location, one of the robots will compute a new meeting location to dynamically update the current agreement and send it to all the sub-team while they wait.
% %
% Finally, when the sub-team receives the updated meeting location, they update the current agreement and increment the pointer to the next agreement.
% %
% The exploration continues until there are no more frontiers to explore. 
% %
% After a robot reaches this stopping criteria, according to its local map, it returns to $q_{start}$ to finalize the exploration.

% In particular, lines $6$, $14$, and $20$ of Algorithm~\ref{alg:smainloop} play an important role during the exploration process, since they demand certain care regarding how $plan$ is generated offline, how to select and explore frontiers dynamically with opportunistic interactions, and how to update and distribute the new $plan$ among a sub-team of robots.

==> DEPRECATED/algorithms/generating_agreements.tex <==
\subsection{Generating Rendezvous Agreements}

To generate the rendezvous $plan$ in line $6$ of Algorithm~\ref{alg:smainloop} we propose a multi-objective optimization, where $K$ and $W$ are variables to be trained. Since is might be difficult to visualize what might happen with the rendezvous plan by simply walking with $K$ and $W$ in a search space, we propose to transpose the problem into an instance of the JSSP (Job-shop Scheduling Problem) and extract metrics, such as how much time robots are exploring, how often they exchange maps, and the connectivity index. As shown in Algorithm~\ref{alg:gen}, the robot responsible for the computation uses these JSSP metrics as an objective function in line $5$ to iterate over the search space. 

\begin{algorithm}
\DontPrintSemicolon
\KwIn{Set of robots $\mathcal{R}$}
\KwOut{Agreement matrix $K$\\
\quad\quad\quad\quad Cost matrix $W$}
\SetKwBlock{Begin}{function}{end function}
\SetKwRepeat{Do}{do}{while}
\Begin($\text{PlanGenerator} {(\mathcal{R})}$) {
    Let $K$ and $W$ be initialized randomly according to the number of robots $|R|$ and constraints;\;
    Let $solution \leftarrow \infty$ be a real number;\;
    \Do{$solution$ is greater than a threshold} {
        Let $\mathcal{I}$ be an instance of the JSSP obtained from $K$ and $W$;\;
        Let $f(\mathcal{I}) = \sum \alpha_ih_i(\mathcal{I}) + \sum \beta_jg_j(\mathcal{I})$ be an objective function composed by metrics $h_i$ and $g_j$ obtained from $\mathcal{I}$, where $\alpha_i$ and $\beta_j$ are normalization factors;\;
        Perform an optimization step on $K$ and $W$ to minimize $f(\mathcal{I})$;\;
        $solution \leftarrow f(\mathcal{I})$;\;
    }
    \Return $K$, $W$;\;
}
\caption{Plan Generator}
\label{alg:gen}
\end{algorithm}

Importantly, in line $5$ of Algorithm~\ref{alg:gen}, we divided the metrics into two summations, and we call them as

\begin{itemize}
    \item \textbf{Plan Behavior Metrics:} $\sum\alpha_ih_i(\mathcal{I})$ tells how often the encounters are going to happen, for how long robots need to explore before attending agreements, and how much area is going to be explored approximately if robots follow the plan.
    \item \textbf{Connectivity Metrics:} $\sum\beta_jg_j(\mathcal{I})$ is used to check if the robots are going to be intermittently connected and is calculated from a proximity graph obtained from $\mathcal{I}$.
\end{itemize}

Next, we present how to generate the JSSP $\mathcal{I}$ from line $4$ and how to calculate the metrics.

\subsubsection{\textbf{Generating the JSSP Instance}}

To extract the metrics from $K$ and $W$ we propose a reduction to the JSSP. In the JSSP there are a set of machines and a set of jobs, where each job has a duration and should be executed by one machine in a specified order. In contrast, the objective of the reduction is to represent each robot as a machine and each job as the task of exploring the environment before attending to a rendezvous agreement. Consequently, each jobs is associated with an agreement from $K$ and its length is influenced by the resources in $W$. The reduction can be accomplish by several different ways, however, the one we propose is presented in Algorithm~\ref{alg:jssp}. Jobs are created in the loops from line $6$ to $15$ and are grouped in line $13$ through the $agreement$ index.

\begin{algorithm}
\DontPrintSemicolon
\KwIn{Set of robots $\mathcal{R}$\\
        \quad\quad\quad Rendezvous agreement matrix $K$\\
        \quad\quad\quad Rendezvous cost matrix $W$}
\KwOut{JSSP instance $I$}
\SetKwBlock{Begin}{function}{end function}
\SetKwRepeat{Do}{do}{while}
\Begin($\text{JSSPReduction} {(\mathcal{R}, K, W)}$) {
    Let $last_{time}$ be a variable that helps to allocate jobs at the correct time;\;
    Let $aux_{time}$ be an auxiliary that helps deciding how much to update $last_{time}$;\;
    Let $\mathcal{I}$ be a set of $|R|$ machines created during the reduction;\;
    \ForEach{$agreement$ row in $K$} {
        $aux_{time} \leftarrow 0$;\;
        \ForEach{$robot$ column in $K[agreement]$} {
            \If{$K[agreement][robot] = 1$} {
                create a new job $job_{new}$ and allocate it to the $jth$ machine in $\mathcal{I}$;\;
                set the starting time of $job_{new}$ as $last_{time}$;\;
                set the length of $job_{new}$ as $W[agreement][robot]$;\;
                set the $job_{new}$ identification as $agreement$;\;
                \If{ending time of $job_{new} > aux_{time}$} {
                    set $aux_{time}$ as the ending time of $job_{new}$;\;
                }
            }
        }
        update $last_{time} \leftarrow aux_{time}$ to allocate the jobs from the next row;\;
    }
    \Return $\mathcal{I}$;\;
}
\caption{Job-shop Scheduling Reduction}
\label{alg:jssp}
\end{algorithm}

\subsubsection{\textbf{Plan Behavior Metrics}}

% The plan behavior metrics are used to measure how often the meet-ups occurs, how many robots participate in the agreements, and for how long they explore before going to the meeting locations. 

From the JSSP instance $\mathcal{I}$, a robot calculates the normalized total number of jobs as

\begin{equation}
\label{eq:num_plans}
h_1(\mathcal{I}) = \mathcal{J}_{\mathcal{I}}(1+\mathcal{J}_{\mathcal{I}})^{-1}
\end{equation}

\noindent
where $J_{\mathcal{I}}$ is the total number of jobs in $\mathcal{I}$; the normalized makespan

\begin{equation}
\label{eq:makespan}
h_2(\mathcal{I}) = max_{\forall t_i \in t_{\mathcal{I}}}(t_i)(1+ max_{\forall t_i \in t_{\mathcal{I}}}(t_i))^{-1}
\end{equation}

\noindent
where $t_{\mathcal{I}}$ is a set containing the finishing time of each machine from $\mathcal{I}$; the normalized standard deviation of the the total idle time $\sigma_{\mathcal{I}}$ between all jobs in $\mathcal{I}$ (i.e., the total time that machines are not processing jobs);

\begin{equation}
\label{eq:sigma_agreement}
h_3(\mathcal{I}) = \sigma_{\mathcal{I}}(1+\sigma_{\mathcal{I}})^{-1}
\end{equation}

\noindent
and the estimated total exploration

\begin{equation}
\label{eq:workdone}
h_4(\mathcal{I}) = (1+\sum_{\text{job}_i \in J_{\mathcal{I}}}job_i\mathcal{E}_j)^{-1}
\end{equation}

\noindent
where $\text{job}_i$ is the length of the $ith$ job from from $\mathcal{I}$ and $\mathcal{E}_j$ is a constant that estimates how much area a robot can explore given the sensor it uses to acquire information to assemble the map (e.g., lidar, sonar, camera) and traveling speed.

% \subsubsection{Metrics Discussion}

% The intuition behind eq. \ref{eq:num_plans} and \ref{eq:makespan} is to quantify how often robots share maps through the number of agreements per time step. Differently, eq. \ref{eq:sigma_agreement} quantifies hows much time the entire team keeps waiting. Finally eq. \ref{eq:workdone} quantifies the expected explored area by all jobs. It also serves as a connection between the generated $plan$, the robot's exploration capabilities, and the bounded area of $\Omega$. Another advantage of associating an expected capability of a robot in eq. \ref{eq:workdone} is that robots can quantify how many times a JSSP instance should be repeated, approximately, to finish exploring $\Omega$ if it is the case. 

% Another insight behind these equations is the fact that the rendezvous agreement $plan$ can be generated whenever needed to encompass updated information about how robots are functioning, however, for the purpose of this research, a robot generates the plan only once. The dynamic part of the $plan$ is related to the meeting locations inside the circular list outside of the $plan$, that are updated dynamically when a sub-team of robots meet.

% It is important to note that the generation of the plan does not aggregate uncertainties besides the expected exploration capability of robots and the bounded size of $\Omega$, however it yielded control over the rendezvous plan that achieved good performances with the exploration policy.

\subsubsection{\textbf{Connectivity Metrics}}

Let $\mathcal{H}$ be a function that generate a condensed proximity graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ that represents each time step in our JSSP instance $\mathcal{I}$. In this graph, vertices are robots and edges represent connectivity. An edge is created between two vertices only if the two robots associated with them if they have a common agreement from $\mathcal{I}$. From $\mathcal{G}$, we propose extracting the connectivity index

\begin{equation}
\label{eq:connectivity_index}
g_1(\mathcal{I}) =  \mathcal{C}(\mathcal{H}(\mathcal{I}))(1 + \mathcal{C}(\mathcal{H}(\mathcal{I})))^{-1}
\end{equation}

\noindent
where $\mathcal{C}(\mathcal{H}(\mathcal{I}))$ is a function that returns the length of the biggest connected component of $\mathcal{H}(\mathcal{I})$. We also propose the utilization of the normalized number of edges

\begin{equation}
\label{eq:edges_count}
g_2(\mathcal{I}) = |\mathcal{E}_{\mathcal{H}(\mathcal{I})}|(1+|\mathcal{E}_{\mathcal{H}(\mathcal{I})}|)^{-1}
\end{equation}

\noindent
where $\mathcal{E}_{\mathcal{H}(\mathcal{I})}$ is the set of edges from $\mathcal{G}$. The intuition behind eq.~\ref{eq:connectivity_index} is to see if the plan makes the robots intermittently share their maps. Additionally, eq.~\ref{eq:edges_count} can be used to count how many robots are inside the same agreement.

% To generate the rendezvous structure, the robot responsible for the computation of the $plan$, in line $6$ of Algorithm~\ref{alg:smainloop}, optimize over the space of possible configurations of $K$ and $W$ to minimize the following multi-objective optimization composed by equations \ref{eq:num_plans} to \ref{eq:edges_count}

% \begin{align}
%     \begin{split}
%      I^* =& \ \underset{\mathcal{I}}{\arg\min} \ (\mu_1 g_1(\mathcal{I}),... , \mu_5 g_5(\mathcal{H}(\mathcal{I})), \mu_6 g_6(\mathcal{H}(\mathcal{I}))) \\
%         & \quad \text{s.t.} \\
%         & g_1(\mathcal{I}), ..., g_6(\mathcal{H}(\mathcal{I})) \geq 0
%     \end{split}
% \end{align}

% \noindent
% where $\{\mu_1, ..,.\mu_6\}$ are importance weights. The intuition behind this optimization is to generate a plan where robots will keep exploring as much as possible at the cost of sharing their maps.

\subsection{Dynamically Updating Agreement Locations}

Differently from the rendezvous agreement plan, the meeting locations are updated dynamically. When a sub-team is attending an agreement, in line $20$ of Algorithm~\ref{alg:smainloop}, the robot with the lowest unique identifier in the sub-team will compute a new meeting location in the $meetup$ variable. It will generate a set of centroids from all the available frontiers from its merged map. Each centroid is calculated considering its K-nearest neighbors given a distance threshold. The robot performing the calculations samples a random centroid from the centroids list and set it as the new $meetup$ for the current agreement. Next, it distributes the new location among all the other robots from the sub-team attending the agreement so they can also update their local variables. Since the system is distributed and we can not ensure that robots will have the same common map, we decided to rely on a random sampling method.




==> DEPRECATED/algorithms/robot_main.tex <==

\section{Robot Simulation Main}

\clearpage

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$robots, rate$}
\KwOut{}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{Main} {(robots)}$) {
    $id \leftarrow GetRobotId()$\;  

    if Leader Create Rendezvous Plan \;
    
    \If{$Consensus(id)$} {
        $inst \leftarrow JSSP(robots, rate)$\;
        $K, W, L \leftarrow SGA(inst)$\;
        $state \leftarrow planning$\;
        $distribute(K,W,L,inst)$\;
    }
    \While{$state \neq finished$} {
        $occ_f, rel \leftarrow Fusion(occ, occ_{near})$\;
        $near \leftarrow CommCheck()$\;
        $state \leftarrow Explore(K, W, L,$ \\ $\quad id, occ_f, rel, state)$\;
    }
}
\caption{Single Robot Main Loop}
\label{alg:mainloop}
\end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$K, W, L, id, occ_f, rel, state$}
\KwOut{$state$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{Explore} {(K, W, L, id, occ_f)}$) {
    \Switch{$state$} {
        \Case{$planning$} {
             $f, z \leftarrow DetectFrontiers(occ_f)$\;
            \If{$|f| > 0$} {
                $choice \leftarrow Str(f, z, near, id, occ_f, rel)$\;
                $state \leftarrow exploring$\;
            } \Else {
                $state \leftarrow finished$\;
            }
        } \Case{$exploring$} {
            $state, fr, p, T \leftarrow Nav(near, state, occ_f,$\\$\quad\quad occ_{new}, res, K, W, id, cur, fr)$\;
        }
        \Case{$rendezvous$} {
            $n \leftarrow GoTo(K[id][cur], occ_f)$\;
            \If{$n = reached$} {
                $state \leftarrow wait$\;
            } \ElseIf{$n = impossible$} {
                $state \leftarrow cycleplan$\;
            }
        } \Case{$wait$} {
            \If{$CheckTimeout(T_{time})$} {
                $state \leftarrow cycleplan$\;
            } \If{$Consensus(id)$} {
                \If{$InRen(K[id][cur])$} {
                    $L \leftarrow UpdateLoc(L, occ_f, K_{items})$\;
                    $state \leftarrow cycleplan$\;
                    $Comm(near, cycleplan)$\;
                } \Else {
                    $Update(T_{time})$
                }
            }
        } \Case {$cycleplan$} {
            $cur \leftarrow Next(K[id][cur], cur)$\;
            $res \leftarrow W[id][cur]$\;
            $fr \leftarrow true$\;
            $state \leftarrow planning$\;
        } \Case {$finisheed$} {
            \If{$GoTo(start, occ_f)$} {
                $state \leftarrow idle$\;
            }
        }
    }
    \Return{$state$}
}
\caption{Single Robot Controller}
\label{alg:mainloop}
\end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$near, state, occ_f, occ_{new}, res, K, W, id, cur, fr$}
\KwOut{$state, fr, p, T$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{Nav} {(.)}$) {
     \If{$Trigger(res, K[id][cur], W[id][cur])$} {
        $state \leftarrow rendezvous$\;
     } \Else {
        \If{$|near| > 0 and fr = false$} {
            $state \leftarrow planning$\;
        } \Else {
            $p \leftarrow ComputePath(choice, occ_f)$\;
            \If{$|p| > 0$} {
                $T \leftarrow OptimizeTrajectory(p)$\;
                \If{$T \neq \emptyset$} {
                    $Execute(T)$\;
                    $UpdateRes(res, occ_f, occ_{new})$\;
                }
            } \If{$Reached(choice)$} {
                $state \leftarrow planning$\;
                $fr \leftarrow false$\;
            }
        }
    }
    \Return{$state, fr, p, T$}
}
\caption{Exploration With Rendezvous}\label{alg:nav}
\end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$occ_f$}
\KwOut{$f, z$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{DetecFrontiers} {(occ_f, q)}$) {
    $c \leftarrow CreateComposition(occ_f)$\;
    $f \leftarrow FilterDetection(c)$\;
    $z \leftarrow \{\}$\;
    \ForEach{$f_i \in f$} {
        $z \leftarrow z \cup {Cost(f_i, q)}$\;
    }
    \Return{$f,z$}
}
\caption{Frontier Detection}\label{alg:frontier}
\end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$f, z, near, id, occ_f, rel$}
\KwOut{$choice$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{Str} {(f, z, near, id, occ_f, rel)}$) {
    \If{$|near| > 0$} {
        $\mathcal{N} \leftarrow NormalFormGame(f, z, near, rel)$\;
        $outcome \leftarrow \arg\max(SW(N))$\;
        $choice \leftarrow ExtractChoice(N[outcome], id)$\;
        \Return{$choice$}
    }
    \Return{$f[\arg\max(z)]$}
}
\caption{Allocation Strategies}
\label{alg:alloc}
\end{algorithm}

\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{$L, occ_f$}
\KwOut{$L$}
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{UpdateLoc} {(L, occ_f, K_{items})}$) {
    $COM \leftarrow \{\}$\;
    \ForEach{$l_i \in L$} {
        \If{$|COM| = 0$} {
            $l_{new} \leftarrow Random(occ_f)$\;
        } \Else {
            $l_{new} \leftarrow MaxDistSample(COM, occ_f, K_{items})$\;
        }
        $COM \leftarrow COM \cup l_{new}$\;
    }
    \Return{$COM$}
}
\caption{Rendezvous KNN Update}
\label{alg:alloc}
\end{algorithm}

\clearpage

%\begin{algorithm}
%\DontPrintSemicolon
%\KwIn{Rendezvous structure $plan$\\
%     \quad\quad\quad Robot unique identifier $id$\\
%     \quad\quad\quad Exploration starting location $q_{start}$}
%\SetKwBlock{Begin}{function}{end function}
%\SetKwRepeat{Do}{do}{while}
%\Begin($\text{StartOnlineExploration} {(plan,id,q_{start})}$) {
%    Let $K$, $W$, and $L$ be the agreement matrix, cost matrix, and locations list obtained from $plan$;\;
%    Let $agreement \leftarrow |L|-1$\ be an integer referencing the current agreement this robot should honor;\;
%    Let $resources$ be the current available resources in the cost matrix at $W[agreement][id]$;\;
%    Let $subteam$ be the participants of the rendezvous agreement at $K[agreement]$;\;
%    Let $location = L[agreement]$ be the current meeting location for this robot;\;
%    Let $state \leftarrow \text{"Explore"}$ be the robot's initial state;\;
    
%    \ForEach {time-step $t$} {   
%        Update occupancy grid $occ$, receive, and merge occupancy grids from nearby robots into $occ$;\;
%        Detect frontiers in $occ$ and store them into $\mathcal{F}$;\;

%        \If{$\mathcal{F}$ is empty} {
%            Navigate to the starting location $q_{start}$;\;
%            \textbf{break};\;
%        }

%        \Switch{$state$} {
%            \Case{\textbf{"Explore"}} {
%                \If{$resources > 0$} {
%                    $Exploration\footnote{This algorithm is expalined in Section...}(\mathcal{F})$;\;
%                } \Else {
%                    $state \leftarrow "SubteamRendezvous"$;\;
%                }
%            } \Case{\textbf{"SubteamRendezvous"}} {
%                Navigate to agreement point $location$;\;
%            \If{$id$ is the lowest from $subteam$ \textbf{and}\\
%                \quad reached $location$ \textbf{and}\\
%                \quad all robots in $subteam$ are at $location$} {
%                    Generate new locations list $L_{new}$;\;
%                    Distribute $L_{new}$ among $subteam$;\;
%                    $L \leftarrow L_{new}$;\;
%                }
%                \uElseIf{received $L_{new}$} {
%                    $L \leftarrow L_{new}$;\;
%                }
%                \If{timeout \textbf{or} $L$ was assigned} {
%                        $agreement =$ \\
%                        \quad\quad $(agreement+1) \mod |L|$;\;
%                        $resources \leftarrow W[agreement][id]$;\; 
%                        $subteam \leftarrow K[agreement]$;\;
%                        $location \leftarrow L[agreement]$;\;
%                        $robotState \leftarrow \text{"Explore"}$;\;
%                }
%            }
%        }
%        \If{explored previously unseen areas\footnote{This algorithm is explained in details in Section...}} {
%            $resources \leftarrow resources - \gamma$;\;
%        }
%    }
%}
%\caption{Robot Online Exploration}
%\label{alg:robotcontroller}
%\end{algorithm}

==> DEPRECATED/algorithms/simplified.tex <==
\section{Methodology}

Our method is grounded in Algorithm~\ref{alg:smainloop}, where an assigned robot formulates a rendezvous agreement plan, that should be followed, and distribute this plan among other robots to start the exploration.
%
When a robot starts the algorithm, it will be assigned an unique identifier and based on this identifier it will compute the rendezvous structure $plan$ or wait until a $plan$ has been received.
%
After all robots have the $plan$ structure, they start the dynamic exploration process for each time-step.

\begin{algorithm}
\DontPrintSemicolon
\SetKwBlock{Begin}{function}{end function}
\Begin($\text{Main} {()}$) {
    Let $q_{start}$ be the starting location;\;
    Let $id$ be an unique identifier $id \in \{0,1,2,3,...\}$ for this robot;\;
    Before the exploration starts, let all robots be waiting and stopped within a communication range from $q_{start}$;\;
    \If{my unique identifier $id$ is $0$} {
        Create a rendezvous agreement structure $plan$;\;
        Distribute $plan$ among all robots through the network with Algorithm~\ref{alg:gen};\;
    } \Else {
        Wait until the rendezvous agreement structure $plan$ have been received;\;
    }
    Let all rendezvous locations specified inside $plan$ be initialized with $q_{start}$;\;
    Let $\mathcal{L}$ be a circular list, where each element is an agreement tuple $(a,l)$
    0.l;\;
    Populate $\mathcal{L}$ with the information from $plan$;\;
    Let the pointer $current$ be the the beginning of $\mathcal{L}$;\;
    before going to the $meetup$ location;\;
    \ForEach{time-step} {
        Receive maps from other nearby robots and merge with my map;\;
        Detect all frontiers from the merged map;\;
        \If{there are no frontiers to explore} {
            \textbf{break};\;
        }
        Explore frontiers if has $resources$ with Algorithm~\ref{alg:robotAlloc};\;
        \If{$resources$ were depleted} {
            Meet a sub-team of all robots in the $meetup$ location, update the $plan$, and $resources$, and $meetup$;\;
        }
    }
    Go back to $q_{start}$;\
}
\caption{Robot Main Procedure}
\label{alg:smainloop}
\end{algorithm}

\subsection{Rendezvous Agreement Plan Structure}

The rendezvous agreement structure $plan$, created with Algorithm~\ref{alg:gen}, is used to help robots decide which other ones to meet and also when this meeting process should start. 
%
We propose to organize the structure of $plan$ through two matrices, $K$ and $W$. Each element of $K$ is a binary number and each element of $W$ is a positive real.
%
We call $K$ as the agreement matrix and $W$ as the cost matrix. The lines of both matrices represent rendezvous agreements and columns represent robots and both are indexed from $0$. For example, consider the following $K$ and $W$ instances,

\begin{align*}
K = \begin{bmatrix}
        1 & 0 & 1\\
        0 & 1 & 1
    \end{bmatrix}
\label{eq:matrices} &&
W = \begin{bmatrix}
        50 & 0 & 100\\
        0 & 100 & 50
    \end{bmatrix}
\end{align*}

\noindent
where, the first line of $K$ tells that the first rendezvous of robot $0$ should be with robot $2$, whereas the second line tells that the first rendezvous of robot $1$ should be with robot $2$.
%
In the aforementioned example, the $W$ matrix is used to tell how much resources each robot should spend before trying to follow the agreements in $K$. 
%
For instance, the first line of $W$ tells that robot $0$ should spend $50$ units of resources exploring the environment before trying to meet with robot $2$ from the agreements specified in the first line of $K$.
%
During Algorithm~\ref{alg:smainloop}, each robot maintains a copy of the $plan$ received at the start of the algorithm and $K$ and $W$ are accessed to create the agreement circular list and also to extract and update the resources in lines $12$ and $20$, respectively.

\subsubsection{Rendezvous Plan}

The $plan$ structure represents several agreements between robots. Each agreement specifies a sub-team of robots that should meet and how much resources each robot in this sub-team should spend before attending to the agreement's location to share maps. 
%
Importantly, each robot can have a different number of agreements and participate in more than one of them. 
%
Before engaging in exploration, robots organize all the agreements they should participate in a circular list with a pointer to its first position.
%
Each element of this list is a tuple $(a,l)$, where $a$ is an index used to reference the agreement inside $plan$ and $l$ its meet-up location. 
%
A robot uses $a$ to help recovering information inside the variable $plan$.
%
The pointer is used by a robot to known which agreement should be attended next. We are going to reference the pointer as \textit{current agreement}.

\subsubsection{Agreement Maintenance}

During the exploration, lines $14$ - $18$ of Algorithm~\ref{alg:smainloop}, robots perform multi-robot exploration by creating a map, merging maps from nearby robots, and selecting frontiers to explore based on which robots are nearby.
%
We explain this exploration process in Algorithm~\ref{alg:robotAlloc}.
%
Differently, line $19$ get the available resources from the current agreement and check if they were spent exploring new areas in the environment.
%
If a robot spent the resources needed to attend to the current agreement's location $l$, it will navigate towards it and wait for the sub-team to arrive.
%
When every robot of the sub-team is at the location, one of the robots will compute a new meeting location to dynamically update the current agreement and send it to all the sub-team while they wait.
%
Finally, when the sub-team receives the updated meeting location, they update the current agreement and increment the pointer to the next agreement.
%
The exploration continues until there are no more frontiers to explore. 
%
After a robot reaches this stopping criteria, according to its local map, it returns to $q_{start}$ to finalize the exploration.

In particular, lines $6$, $14$, and $20$ of Algorithm~\ref{alg:smainloop} play an important role during the exploration process, since they demand certain care regarding how $plan$ is generated offline, how to select and explore frontiers dynamically with opportunistic interactions, and how to update and distribute the new $plan$ among a sub-team of robots.

==> DEPRECATED/comments.tex <==

% \textcolor{blue}{At each time step, a robot $i$ receive maps from others within its communication range} \thales{this is confusing and imply there's always a robot withing comm range of i.} \sugthales{In a nutshell, the exploration is as follow: at any time step a robot $i$ can receive map from another robot within its communication range, then} \sout{to} perform map merging with its local map and assemble its current state $s_i(t)$ to execute its policy.
% %
% \sout{It} \sugthales{The robot} explores the environment by selecting and executing actions from $\sugthales{\mathcal{A}}_i\sout{A} $, considering the frontiers obtained from its merged map.
% %
% When exploring, it constantly updates its path and trajectory to account for localization and mapping uncertainties.
% %
% We propose extending $A_i$ with a controller that is also responsible for handling the fulfillment of agreements. 
% %
% An action from this controller allows a robot to navigate towards the location associated with the sub-team \ani{Is this a sub-team or a sub-team member?}\alysson{a sub-team} it should meet, share maps, update the rendezvous location or plan, and wait at the rendezvous location (see Fig.~\ref{fig:execution} components highlighted in light blue).
% %
% In particular, once at a rendezvous location, a robot waits until the sub-team it should meet arrives or until a timeout.
% %
% After the meeting, one of the robots participating selects a new rendezvous location and sends it to the sub-team from the meeting.
% %
% % \ani{I am confused.  I thought the robot's hold the agreements.  How are they going to send their agreement to their sub-team if they are not connected?  And how does an agreement have a sub-team?}.
% %
% In the case of a timeout, robots select the next agreement they should fulfill and start exploring again.

==> DEPRECATED/gazebo.tex <==
\subsubsection{Gazebo Simulations}

We deployed our method in non-holonomic robots using Gazebo, and we let them perform Simultaneous Localization and Mapping (SLAM) \cite{Dissanayake2001} with the gmapping package. We set our communication range to $2$m and stitch their maps when they can communicate. We designed a safety heuristic that reduces the robot's velocities when near each other to prevent accidents in rendezvous zones. Our robots navigate with Roadmaps and a local planner based on Artificial Potential Fields \cite{Warren1989}. We simplified KNN, eq.~\ref{eq:frontier_utility}, and picked rendezvous updates for this deployment. We evaluated the agreement behavior in $4$ different trials.

Fig.~\ref{fig:trajectories}, shows the overlayed trajectories of robots when executing the rendezvous agreements. We observed that the communication between robots in ROS made the integration significantly harder, and we had to design a synchronization mechanism to coordinate robots in their corresponding rendezvous agreement. Particularly, trial $1$ was the most difficult to accomplish, and we had to intervene due to rendezvous locations close to each other. Nevertheless, we show that the deployment is feasible and that we could coordinate the agreements in a distributed manner with ROS.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/results/trials/trials.png}
    \caption{Traffic in rendezvous zones for $4$ trials in Gazebo simulation while executing intermittent rendezvous agreements. White circles are rendezvous locations and colored lines are trajectories.}
    \label{fig:trajectories}
    \vspace{-2.0em}
\end{figure}

==> DEPRECATED/method_-_frontier_exploration.tex <==
\section{Experimental Configuration}

\subsection{Frontier Exploration with Rendezvous Prioritization}
\label{sec:frontier_based_rendezvous}

Each robot $r_i$ has its cell decomposition $\mathcal{C}_i$ obtained from $\Omega$ that can be shared with others when able to communicate and is used for planning. We will assume that a robot must find a shortest-length path $\delta(f_i)$ in $\mathcal{C}_i$ to navigate towards a frontier $f_i$ with local and global planners. 

We propose to prioritize\footnote{The cosine between the vectors can lead to inefficient exploration, and we recommend increasing $\beta$ until reaching the expected behavior.} regions in $\Omega$ to explore by considering the rendezvous locations in $l$ when robots are exploring. Let $x$ be the last rendezvous location of the synchronization point, $y$ be the rendezvous location of the current agreement of a robot. We define the reward of visiting a frontier $f_i$ through the following function

\begin{equation}
\label{eq:frontier_utility}
u(f_i) = \alpha \frac{\mathcal{N}_{f_i}}{\Phi(f_i)} + \beta \langle\Vec{xf_i}, \Vec{yf_i} \rangle
\end{equation}

\noindent
where $\mathcal{N}_{f_i}$ is the total uncovered area while the robot is following $\delta(f_i)$, $\Phi(f_i)$ is the path length, $\Vec{xf_i} = (f_i - x)$, and $\Vec{yf_i} = (f_i - y)$. We use $\alpha$ and $\beta$ as scalars to regulate each term's importance. In Fig.~\ref{fig:dynamic_update}, we highlight the prioritized regions of $\Omega$ for each agreement in a rendezvous plan with locations $l_1$ to $l_4$. If the current agreement location of a robot is $l_1$, then it will prioritize the region highlighted with the same color as the rendezvous location. During the exploration, our method follows two strategies to select frontiers to explore, \textit{Local Coordination} and \textit{Multi-robot Coordination}, and we describe them as follows.

\subsubsection{Local Coordination Strategy}
\label{sec:local_coord}

Let $\mathcal{D}$ be a set, such that each of its elements is a tuple $(f_{i}, u_i)$, where $f_{i}$ is a frontier and $u_i := u(f_i)$ its associated utility. A robot $r_i$ follows the local coordination strategy if there are no other robots in its communication range by finding the most promising frontier as $\{(f_{i}, u_i) \in \mathcal{D}: u_i \geq u_j \ \forall \ {(f_{j}, u_j)} \in \mathcal{D} \}$ and tries to navigate towards it using the path $\delta(f_i)$.



\subsubsection{Multi-robot Coordination Strategy}
\label{sec:multi_coord}

Otherwise, if other robots are in the range of communication of $r_i$, we coordinate them in a distributed manner by maximizing the local \textit{Social Welfare}. We define the local Social Welfare as a choice from $A$ where each robot nearby $r_i$ simultaneously selects a frontier to explore. Consider $\mathcal{O} = \mathcal{F}_{b} \times ... \times \mathcal{F}_{z}$ as the set of all possible outcomes, where $o_j \in \mathcal{O}$ is a tuple containing the frontiers each nearby robot $\{r_b,...,r_z\}$ should select. We approximate $\max\sum_{f \in o_j} u(f), \forall \ o_j \in \mathcal{O}$ and assign each frontier from this outcome to each robot involved in the calculation. To do this assignment, we designed a consensus algorithm based on unique identifiers. Importantly, we penalize all rewards tied to frontiers at the same location with a negative weight to prevent redundancy. 

==> DEPRECATED/tables_kbp.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{ clllllllllllll }
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{Philly}} &
  \multicolumn{1}{c}{\centering{NY}} &
  \multicolumn{1}{c}{\centering{DC}} &
  \multicolumn{1}{c}{\centering{Tokyo}} &
  \multicolumn{1}{c}{\centering{Beijing}} & 
  \multicolumn{1}{c}{\centering{Dubai}} &
  \multicolumn{1}{c}{\centering{Moscow}} &
  \multicolumn{1}{c}{\centering{Berlin}} &
  \multicolumn{1}{c}{\centering{Lisbon}} &
  \multicolumn{1}{c}{\centering{London}} &
  \multicolumn{1}{c}{\centering{Paris}} & 
  \multicolumn{1}{c}{\centering{Rio}} \\ \cline{1-13}
\multicolumn{1}{c|}{CSBS} &
  \multicolumn{1}{l|}{\small${6760\pm 660}$} &
  \multicolumn{1}{l|}{\small${4297\pm 606}$} &
  \multicolumn{1}{l|}{\small${6841\pm 1221}$} &
  \multicolumn{1}{l|}{\small${6034\pm 999}$} &
  \multicolumn{1}{l|}{\small${6137\pm 883}$} &
  \multicolumn{1}{l|}{\small${8336\pm 1214}$} &
  \multicolumn{1}{l|}{\small${7069\pm 1119}$} &
  \multicolumn{1}{l|}{\small${7337\pm 827}$} &
  \multicolumn{1}{l|}{\small${4984\pm 521}$} &
  \multicolumn{1}{l|}{\small${6583\pm 954}$} &
  \multicolumn{1}{l|}{\small${6257\pm 867}$} &
  \multicolumn{1}{l}{\small${7367\pm 1120}$} \\ \cline{1-13} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${5969\pm 622}$} &
  \multicolumn{1}{l|}{\small${3644\pm 597}$} &
  \multicolumn{1}{l|}{\small${6426\pm 845}$} &
  \multicolumn{1}{l|}{\small${5637\pm 903}$} &
  \multicolumn{1}{l|}{\small${5884\pm 886}$} &
  \multicolumn{1}{l|}{\small${7647\pm 1375}$} &
  \multicolumn{1}{l|}{\small${7333\pm 1128}$} &
  \multicolumn{1}{l|}{\small${6096\pm 746}$} &
  \multicolumn{1}{l|}{\small${4895\pm 1035}$} &
  \multicolumn{1}{l|}{\small${5777\pm 956}$} &
  \multicolumn{1}{l|}{\small${5629\pm 669}$} &
  \multicolumn{1}{l}{\small${6089\pm 773}$} \\ \cline{1-13}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${5699\pm 680}$} &
  \multicolumn{1}{l|}{\small${3337\pm 421}$} &
  \multicolumn{1}{l|}{\small${6034\pm 652}$} &
  \multicolumn{1}{l|}{\small${5116\pm 558}$} &
  \multicolumn{1}{l|}{\small${5693\pm 751}$} &
  \multicolumn{1}{l|}{\small${6850\pm 810}$} &
  \multicolumn{1}{l|}{\small${5852\pm 968}$} &
  \multicolumn{1}{l|}{\small${6154\pm 824}$} &
  \multicolumn{1}{l|}{\small${4754\pm 811}$} &
  \multicolumn{1}{l|}{\small${5500\pm 915}$} &
  \multicolumn{1}{l|}{\small${5453\pm 712}$} &
  \multicolumn{1}{l}{\small${6063\pm 828}$} \\ \cline{1-13} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small$\mathbf{4083\pm 403}$} &
  \multicolumn{1}{l|}{\small$\mathbf{2668\pm 189}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4137\pm 244}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4030\pm 297}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3986\pm 322}$} &
  \multicolumn{1}{l|}{\small$\mathbf{5150\pm 505}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4034\pm 368}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4276\pm 364}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3202\pm 234}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3925\pm 163}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4417\pm 382}$} &
  \multicolumn{1}{l}{\small$\mathbf{4108\pm 470}$} \\ \cline{1-13} 
  
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{prk01}} &
  \multicolumn{1}{c}{\centering{prk02}} &
  \multicolumn{1}{c}{\centering{prk03}} &
  \multicolumn{1}{c}{\centering{prk04}} &
  \multicolumn{1}{c}{\centering{air01}} &
  \multicolumn{1}{c}{\centering{air02}} &
  \multicolumn{1}{c}{\centering{air03}} &
  \multicolumn{1}{c}{\centering{air04}} &
  \multicolumn{1}{c}{\centering{cons01}} &
  \multicolumn{1}{c}{\centering{cons02}} &
  \multicolumn{1}{c}{\centering{cons03}} &
  \multicolumn{1}{c}{\centering{cons04}} \\ \cline{1-13}
\multicolumn{1}{c|}{CSBS} &
  \multicolumn{1}{l|}{\small${5937\pm 971}$} &
  \multicolumn{1}{l|}{\small${1799\pm 305}$} &
  \multicolumn{1}{l|}{\small${4933\pm 1109}$} &
  \multicolumn{1}{l|}{\small${2692\pm 461}$} &
  \multicolumn{1}{l|}{\small${4059\pm 390}$} &
  \multicolumn{1}{l|}{\small${6237\pm 686}$} &
  \multicolumn{1}{l|}{\small${4452\pm 545}$} &
  \multicolumn{1}{l|}{\small${5488\pm 999}$} &
  \multicolumn{1}{l|}{\small${7308\pm 1126}$} &
  \multicolumn{1}{l|}{\small${4628\pm 790}$} &
  \multicolumn{1}{l|}{\small${5340\pm 927}$} &
  \multicolumn{1}{l}{\small${3865\pm 407}$} \\ \cline{1-13} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${5756\pm 826}$} &
  \multicolumn{1}{l|}{\small${1709\pm 291}$} &
  \multicolumn{1}{l|}{\small${4830\pm 881}$} &
  \multicolumn{1}{l|}{\small${2775\pm 449}$} &
  \multicolumn{1}{l|}{\small${4049\pm 271}$} &
  \multicolumn{1}{l|}{\small${5739\pm 710}$} &
  \multicolumn{1}{l|}{\small${4584\pm 453}$} &
  \multicolumn{1}{l|}{\small${5006\pm 618}$} &
  \multicolumn{1}{l|}{\small${6682\pm 912}$} &
  \multicolumn{1}{l|}{\small${4215\pm 474}$} &
  \multicolumn{1}{l|}{\small${4779\pm 601}$} &
  \multicolumn{1}{l}{\small${3378\pm 337}$} \\ \cline{1-13}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${5379\pm 533}$} &
  \multicolumn{1}{l|}{\small${1726\pm 349}$} &
  \multicolumn{1}{l|}{\small${4114\pm 479}$} &
  \multicolumn{1}{l|}{\small${2948\pm 481}$} &
  \multicolumn{1}{l|}{\small${3790\pm 288}$} &
  \multicolumn{1}{l|}{\small${5692\pm 561}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4298\pm 330}$} &
  \multicolumn{1}{l|}{\small${4959\pm 454}$} &
  \multicolumn{1}{l|}{\small${6188\pm 900}$} &
  \multicolumn{1}{l|}{\small${4126\pm 535}$} &
  \multicolumn{1}{l|}{\small${4608\pm 527}$} &
  \multicolumn{1}{l}{\small${3009\pm 381}$} \\ \cline{1-13} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small$\mathbf{3603\pm 389}$} &
  \multicolumn{1}{l|}{\small$\mathbf{1624\pm 181}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3363\pm 362}$} &
  \multicolumn{1}{l|}{\small$\mathbf{2307\pm 298}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3572\pm 394}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4812\pm 639}$} &
  \multicolumn{1}{l|}{\small${4327\pm 489}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4137\pm 424}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4406\pm 418}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3362\pm 230}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3908\pm 524}$} &
  \multicolumn{1}{l}{\small$\mathbf{2827\pm 361}$} \\ \cline{1-13} 
\end{tabular}
}
\caption{Benchmark results for our dataset composed of cities, parking lots (prk), airport sections (air), and constructions sites (cons). }
\label{tab:table_cities}
\vspace{-1.5em}
\end{table*}


==> sections/BACKUP-2-background_and_problem.tex <==
\section{Background}
\label{sec:problem_statement}

\subsection{Notation}

In the MRE application, we denote an unknown bounded environment as $\Omega \subset \mathbb{R}^2$. Individual robots are denoted by the subscript $i$, where $\mathcal{R} = \{1, \ldots, n\}$ represents the set of $n$ robots. At each time step $t$, $m_i(t)$ denotes the local map built by robot $i$, $\mathcal{F}_i(t)$ denotes the frontier set built by robot $i$ from its map $m_i(t)$, $q_i(t)$ denotes the position and orientation of robot $i$, $s_i(t)$ denotes the robot $i$ current state, $\mathcal{A}_i$ and $\mathcal{A}_i(t)$ denotes the action space and the action space at a time step $t$ for robot $i$, and $a_i(t)$ denotes the action taken by robot $i$. We use the variable $\phi$ to represent the maximum allowable distance for communication. Consider that the union operator over maps $\bigcup_i m_i(t)$ provides map merging with appropriate transformations.

\subsection{Multi-robot Exploration and Intermittent Connectivity}

In classic multi-robot frontier exploration, a set of $n$ robots $\mathcal{R}$ explore an unknown bounded environment $\Omega$. A robot $i$ perceives the environment, builds a local map $m_i(t)$, estimates its pose $q_i(t)$, and constructs the frontier set $\mathcal{F}_i(t)$ at each time step $t$. It then explores by maintaining its current state $s_i(t)$, represented by the tuple $(\mathcal{R}_i(t), m_i(t), q_i(t))$, and taking appropriate actions. An action $a_i(t) \in \mathcal{A}_i(t)$ is the process of calculating and updating a path towards a location from $\Omega$, and following the path. For frontier exploration, each action is associated with a frontier that robot $i$ can explore or a location where robots should meet. We define the utility of an action as $u_i(a_i(t))$, which reflects the benefit of navigating towards the location associated with $a_i(t)$ considering the associated path cost. To coordinate exploration among multiple robots, a task allocation algorithm \cite{Bramblett2022} helps select frontiers that maximize the sum of the robots' utility functions.

We model the connectivity among robots at a time step $t$ as a graph $\mathcal{G}(t) = (\mathcal{R}, \mathcal{E}(t))$, where an edge $e(t) = (i, j)$ from $\mathcal{E}(t)$ represents the connectivity between robots $i$ and $j$. We use a communication model based on a communication range $\phi$. Therefore, we consider the distance between two robots to establish a communication link. At each time step $t$, an edge $e(t)$ between robots $i$ and $j$ exists only if $||q_i(t) – q_j(t)|| \leq \phi$, where $q_i(t)$ is the configuration of robot $i$. Importantly, we also define a sub-team of robots as a sub-team as a set of two or more robots that eventually and periodically meet $\mathcal{T}_s=\{i: \forall\ i\in \mathcal{T}_s, \exists\ j\in \mathcal{T}_s,\exists\ \hat{t}\mathrm{~such~that~} (i,j)\in \mathcal{E}(\hat{t}) \}$. Robots are intermittently connected if the union of the graphs $\{\mathcal{G}(a),\ldots,\mathcal{G}(b)\}$ forms a connected graph for every $b-a$ steps. Map merging enhances efficiency, allowing a robot to receive and integrate a map $m_j(t)$ from other robot within its communication range $\phi$ into $m_i(t)$, such that $m_i(t+1) = \bigcup_j m_j(t)$ for all received $m_j(t)$. Exploration continues until the union of all frontier sets $\bigcup_t \mathcal{F}_i(t)$ is empty.

\subsection{DEC-POMDP and Problem Statement}

The underlying DEC-POMDP of the MRE application is defined as the tuple $(\mathcal{R}, \mathbb{S}, \mathbb{A}, T, \mathbb{O}, O, R)$, where $\mathbb{S}$ is a set of all possible joint states, $\mathbb{A}$ is a set of joint actions, $T$ is the set of conditional transition probabilities, $\mathbb{O}$ is the set of joint observations, $O$ is the set of observations probabilities, $R$ is the immediate reward. For simplicity, we omitted the horizon and the initial system's conditions. We define a joint state $s(t) \in \mathbb{S}$ as $(s_1(t),\ldots,s_n(t))$ and a joint action as $a(t) \in \mathbb{A}$ as $(a_1(t),\ldots,a_n(t))$, where $\mathbb{A} = \mathcal{A}_1 \times \ldots \times \mathcal{A}_n$. Differently, a joint observation $o(t) \in \mathbb{O}$ is defined as $o(t) = s(t)$ at a time step $t$, and its probability is given by $O(o(t)|a(t),s(t+1))$. The transition and observation probabilities are usually unknown for the MRE application, and the true state of the system can not be measured due to localization and mapping uncertainties. 

The immediate reward $R : \mathbb{A} \times \mathbb{S} \rightarrow \mathbb{R}$ is function that associates actions and states to real numbers, and we define the \textit{return} of the DEC-POMDP as a bounded sum $\sum_t R(s(t), a(t))$ because $\Omega$ has a limited number of frontiers that can be explored. For the MRE application, we approximate the reward $R(s(t), a(t))$ as the utility sum of the actions $\sum_i u_i(a_i(t))$ from the joint action $a(t)$. In this regard, a joint policy can be represented as $\pi = \{\pi_1,...\pi_n\}$, where $\pi$ is decentralized and each $\pi_i$ is a finite state controller \cite{Amato2013} that aims at maximizing the return through $a(t)$. From the perspective of a decentralized policy, robots are unaware of the joint state $s(t)$, joint action $a(t)$, joint observation $o(t)$, and the return is available only during the planning phase.

\begin{problem}[MRE Problem with Intermittent Rendezvous]
Design a set of decentralized robot controllers $\pi = \{\pi_1,...,\pi_n\}$, where each controller $\pi_i$ directs robot $i$ to explore frontiers from $\mathcal{F}_i(t)$ through joint actions $a(t)$. Ensure that the union of the graphs of the connectivity graphs $\{\mathcal{G}(a),\ldots,\mathcal{G}(b)\}$ is connected for every $b-a$ steps until $\bigcup^{\mathcal{T}+1}_i \mathcal{F}_i(t) = \emptyset$. The objective is to maximize the return of the DEC-POMDP, defined as $\sum_t\sum_i u_i(a_i(t))$, where $a_i(t)$ represents the action of robot $i$ in the joint action $a(t)$. At each time step, robots operate based on their individual states $s_i(t)$ and are unaware of the joint state $s(t)$, joint actions $a(t)$, and joint observations $o(t)$.
\end{problem}



==> sections/BACKUP-3-method-rendezvous-backtup.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE EXECUTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/figures_tex/2-figure_diagram}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE EXECUTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Methodology}

Our method for frontier exploration with intermittent rendezvous is depicted in fig.~\ref{fig:execution}.
%
Before exploring, one robot from $\mathcal{R}$ calculates an initial rendezvous plan for the team, considering an estimate about the area of $\Omega$ and the robots' sensing and traveling speed.
%
The plan estimates how sub-teams of robots should rendezvous during the MRE mission.
%
Robots can update the plan later to account for new information. 

%\ani{So the initial plan is computed centrally? This is fine.}
%
% :)
%
% if they have the same q_i as a starting point, there is no reason not to exploit the fact that they have global information at t=0 and that $\bigcup_i m_i(t=0)$, since this conveys important information about the initial setup

We define the plan through agreements between robots, where an agreement represents a contract that they should fulfill when exploring (see fig.~\ref{fig:agreements} \ani{Be consistent.  Either use Fig. or fig. but not both.}).
%
Agreements specify which sub-team of robots should meet and how many time steps from $\mathcal{T}$ each robot must explore before going to an assigned rendezvous location. \ani{When you say sub-team, does it mean you want 2 robots to meet up for each rendezvous?  Or do you mean more than 2 robots must meet up during each rendezvous?  How is this being specified mathematically?}
%
To fulfill an agreement, each robot from the sub-team should meet at their rendezvous location and share maps. 
%
In contrast, robots update their sub-team rendezvous location or the plan after fulfilling an agreement, and they are fulfilled from the first to the last.
%
For example, before fulfilling the $2^{nd}$ agreement, robot $2$ should fulfill the $1^{st}$ one. \ani{Why do we not have a definition for each robot's contract set?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE agreements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/figures_tex/3-figure_agreements}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE agreements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A robot $i$ may receive maps from others within its communication range to perform map merging with its local map when executing its policy.
%
It explores the environment by selecting and executing actions from $A_i$, considering the frontiers obtained from its merged map.
%
When exploring, it constantly updates its path and trajectory to account for localization and mapping uncertainties.
%
We propose extending $A_i$ with a controller that is also responsible for handling the fulfillment of agreements. 
%
An action from this controller allows a robot to navigate towards the location associated with the sub-team \ani{Is this a sub-team or a sub-team member?} it should meet, share maps, update the rendezvous location or plan, and wait at the rendezvous location (see fig.~\ref{fig:execution} components highlighted in light blue).
%
In particular, once at a rendezvous location, a robot waits until the sub-team it should meet arrives or until a timeout.
%
After the meeting, one of the robots participating selects a new rendezvous location and sends it to the agreement's sub-team \ani{I am confused.  I thought the robot's hold the agreements.  How are they going to send their agreement to their sub-team if they are not connected?  And how does an agreement have a sub-team?}.
%
In the case of a timeout, robots select the next agreement they should fulfill and start exploring again.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE JSSP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/figures_tex/4-figure_jssp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE JSSP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Generating the Rendezvous Plan}

We propose an agreement matrix $K$ and the steps matrix $W$ to represent the plan efficiently.
%
Each element of $K$ is a binary number, and each element of $W$ is a positive real. 
%
The rows of both matrices represent rendezvous agreements, and columns represent robots. 
%
For example, the following $K$ and $W$ instances represent the agreements from fig.~\ref{fig:agreements}~\ani{Based on your figure, it looks like Robot 1 participates in the 1st, 3rd, and 4th agreement but your caption doesn't seem to reflect the picture.}, 
%\vspace{-0.5em}
\begin{align*}
K = \begin{bmatrix}
        1 & 1 & 0\\
        0 & 1 & 1 \\
        1 & 0 & 1 \\
        1 & 1 & 0
    \end{bmatrix}
\label{eq:matrices} &&
W = \begin{bmatrix}
        50 & 50  & 0\\
        0  & 50  & 100 \\
        90 & 0   & 40 \\
        50 & 100 & 0
    \end{bmatrix}
\end{align*}

\noindent
where, the first line of $K$ tells that the first rendezvous of robot $1$ should be with robot $2$, whereas the second line tells that the first rendezvous of robot $3$ should be with robot $2$. 
%
Since agreements are fulfilled from the first to the last, this example implies that robot $3$ has to explore until robot $2$ fulfills its first agreement.
%
The $W$ matrix tells how many time steps each robot should explore before fulfilling an agreement from $K$. 
%
For instance, the first line of $W$ tells that robots $1$ must explore for $50$ time steps before meeting with robot $2$.
%
Importantly, the rendezvous locations are associated with the sub-teams, that can meet at different moments, and not agreements.


While $K$ and $W$ are compact representations that can be deployed into robots with little computational cost, seeking a solution that reduces waiting times in their domain might be inefficient.
%
Consequently, to generate the matrices, we propose transforming $K$ and $W$ into a JSSP instance $\mathcal{I}$ and evaluating metrics such as the \textit{Makespan}.
%
In this work, we particularly designed Algorithm~\ref{alg:gen} inspired on Evolutionary Computing \cite{Zou2024} to generate them \ani{What are you generating?  And is Algorithm 1 just a genetic algorithm solution to the JSSP?} .
%
It transforms many candidate matrices pairs $W_i$ and $K_i$ from a population into instances $\mathcal{I}_i$ of the JSSP (see fig.~\ref{fig:jss_instance}) and uses the multi-objective function $z(\mathcal{I})$ to calculate their value.
%
After evaluating each solution, it creates a new population and applies the \textit{mutation} function over them, where it automatically regulates the number of agreements in the plan by randomly adding or removing them from $K_i$.
%
Finally, the algorithm sets the new population and repeats until reaching a stopping criterion.

\begin{algorithm}[t!]
\small
\DontPrintSemicolon
\KwIn{Number of robots $|\mathcal{R}|$}
\KwOut{Agreement matrix $K$\\
\quad\quad\quad\quad Cost matrix $W$}
\SetKwBlock{Begin}{function}{end function}
\SetKwRepeat{Do}{do}{while}
\Begin($\text{PlanGenerator} {(|\mathcal{R}|)}$) {
    Initialize a random population $\mathcal{P}$ where each individual is a pair $K_i$ and $W_i$, given the number of robots $|\mathcal{R}|$;\;
    $solution \leftarrow \emptyset$;\;
    \Do{not meeting stopping criterion} {
        Transform each pair $K_i$ and $W_i$ from $\mathcal{P}$ into a JSSP instance $\mathcal{I}_i$;\;
        Let $z(\mathcal{I}) = \sum \alpha_ah_a(\mathcal{I}) + \sum \beta_bg_b(\mathcal{I})$ be an objective function composed by metrics $h_a$ and $g_b$ obtained from $\mathcal{I}$, where $\alpha_a$ and $\beta_b$ are weights;\;
        Evaluate each $\mathcal{I}_i$ with $z(\mathcal{I}_i)$;\;
        Do \textit{selection}, \textit{crossover}, and \textit{mutation}, and create a new population, where each individual is a pair $K_j$ and $W_j$;\;
        Assign the new population to $\mathcal{P}$;\;
        $solution \leftarrow \argmaxnew_{\mathcal{I}_i} z(\mathcal{I}_i)$;\;
    }
    Extract $K$ and $W$ from $solution$;\;
    \Return $K$, $W$;\;
}
\caption{\small{Plan Generator}}
\label{alg:gen}
\end{algorithm}

\begin{algorithm}[t!]
\small
\DontPrintSemicolon
\KwIn{Number of robots $|\mathcal{R}|$\\
        \quad\quad\quad Rendezvous agreement matrix $K$\\
        \quad\quad\quad Rendezvous exploration steps matrix $W$}
\KwOut{JSSP instance $I$}
\SetKwBlock{Begin}{function}{end function}
\SetKwRepeat{Do}{do}{while}
\Begin($\text{JSSP} {(|\mathcal{R}|, K, W)}$) {
    Let $\mathcal{I}$ be a set of $|R|$ machines;\;
    \ForEach{$agreement$ row in $K$} {
        \ForEach{$robot$ column in $K[agreement]$} {
            \If{$K[agreement][robot] = 1$} {
                create a new job $job_{new}$ and allocate it to the $jth$ machine in $\mathcal{I}$;\;
                set the length of $job_{new}$ as $W[agreement][robot]$ and update its starting and ending times according to what was already allocated to the $jth$ machine;\;
                mark $job_{new}$ as belonging to $agreement$ to help to recover $K$ and $W$ through the inverse process;\;
            }
        }
    }
    \Return $\mathcal{I}$;\;
}
\caption{\small{Job-shop Scheduling Transformation}}
\label{alg:jssp}
\end{algorithm}


Line $5$ of Algorithm~\ref{alg:gen} creates the JSSP instance $\mathcal{I}_i$, which contains a set of machines (robots) and a set of jobs (sub-task of exploring the environment before fulfilling an agreement), where each job has a duration and belongs to a machine.
%
The details about the transformation are explained in Algorithm~\ref{alg:jssp}, which creates and inserts jobs into $\mathcal{I}_i$ by iterating over lines of $K_i$. 
%
At the same time, it uses the values from the steps matrix $W_i$ and the length of the jobs already inserted into $\mathcal{I}_i$ to adjust their starting and ending times.
%
A group of jobs is virtually created at line $8$ of Algorithm~\ref{alg:gen} to represent an agreement from $K_i$ as defined in fig.~\ref{fig:jss_instance}.

Importantly, we divided the objective function $z(\mathcal{I})$ at line $6$-$7$ of Algorithm~\ref{alg:gen} into the following terms:

\begin{itemize}
    \item \textbf{Plan Behavior Error:} $\sum\alpha_ah_a(\mathcal{I})$ is used to generate plans considering an estimate of how big is $\Omega$ with minimum waiting times and an agreement fulfillment frequency.
    \item \textbf{Connectivity Metrics:} $\sum\beta_bg_b(\mathcal{I})$ is used to check if the robots are going to be intermittently connected if they follow the plan.
\end{itemize}


\subsubsection{Plan Behavior Error}
\label{sec:planerr}

From the JSSP instance $\mathcal{I}$, the algorithm calculates the exploration estimate error,

\begin{equation}
\label{eq:workdone}
h_1(\mathcal{I}) = ((\Omega_A - \Omega_E) - \sum_{\text{job}_i \in J_{\mathcal{I}}}job_i\mathcal{X}_j)^2
\end{equation}

\noindent
where, $(\Omega_A - \Omega_E)$ is an estimate of how much area is left to explore, given its estimated size $\Omega_A$, and what robots already explored $\Omega_E$, $job_i$ is the length of the $ith$ job, and $\mathcal{X}_j$ is a constant that estimates how much area a robot can explore, given the sensor it uses to acquire information from $\Omega$ ({\it e.g.}, lidar, sonar, camera) and traveling speed; the work done error,
\vspace{-0.5em}
\begin{equation}
\label{eq:desired}
h_2(\mathcal{I}) = (\sum_{\text{job}_i \in J_{\mathcal{I}}}job_i - \sum_{\text{job}_i \in J_{\mathcal{I}}}(job_i + \mathcal{Y}(job_i)))^2
\end{equation}

\noindent
where, $job_i$ is the job length and $\mathcal{Y}(job_i)$ is the number of time steps that should be added to reduce waiting times at rendezvous locations; and the deviation between rendezvous encounters,

\begin{equation}
\label{eq:sigma_agreement}
h_3(\mathcal{I}) = \sqrt{\frac{1}{|\mathcal{J}_{\mathcal{I}}|}\sum_{job_{i} \in \mathcal{J}} (job_i - \bar{job})^2}
\end{equation}

\noindent
where, $job_i$ is the job length, $|\mathcal{J}_{\mathcal{I}}|$ is the number of jobs from $\mathcal{I}$, and $\bar{job}$ is the average job length.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE Proximity graphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/figures_tex/5-figure_proximity_graph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE Proximity graphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsubsection{Connectivity Metrics}
\label{sec:connecterr}

Let $\mathcal{H}_{\mathcal{I}}$ be a set of proximity graphs obtained from a JSSP instance $\mathcal{I}$ as exemplified in fig.~\ref{fig:prox_graph}.
%
We propose creating a new graph $\mathcal{G}_{dense}$, which is a condensed version of all graphs in $\mathcal{H}_{\mathcal{I}}$ to calculate the connectivity metrics.
%
Each vertex from $\mathcal{G}_{dense}$ is a robot, and an edge exists between robots $r_i$ and $r_j$ from $\mathcal{G}_{dense}$ if any of the proximity graphs from $\mathcal{H}(\mathcal{I})$ connects them at a time interval.
%
From $\mathcal{G}_{dense}$, we propose extracting the connectivity index,

\begin{equation}
\label{eq:connectivity_index}
g_1(\mathcal{I}) = 1 - \frac{1}{1 + \mathcal{C}(\mathcal{G}_{dense})}
\end{equation}

\noindent
where, $\mathcal{C}(\mathcal{G}_{dense})$ is a function that returns the length of the biggest connected component of $\mathcal{G}_{dense}$. We also propose extracting,

\begin{equation}
\label{eq:edges_count}
g_2(\mathcal{I}) = |\mathcal{E}'|
\end{equation}

\noindent
where, $|\mathcal{E}'|$ is the number of edges from $\mathcal{G}_{dense}$. 
%
The intuition behind the number of edges is to avoid over-connectivity.
%
In addition, Equations~\ref {eq:connectivity_index} and \ref{eq:edges_count} can be easily adapted to verify the connection between disjoint time intervals.

==> sections/figures_tex/4-figure_jssp.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/JSSP.png}
    \caption{Gantt diagram from a JSS instance of a rendezvous plan from the agreements from fig.~\ref{fig:agreements}. The important components are the agreements (contract between robots), the agreement fulfillment (a rendezvous encounter), the jobs and their meaning (what robots do during the execution of a job), and allocation shifts that may happen when generating the plan (the time robots wait for others).}
    \label{fig:jss_instance}
    \vspace{-2.0em}
\end{figure*}

==> sections/figures_tex/5-figure_proximity_graph.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/connectivity_graph.png}
    \caption{Proximity graphs for the JSSP instance from fig.~\ref{fig:jss_instance}. Sub-teams of robots 1-3 should be connected after finishing their jobs, according to the proximity graphs at the top, because they will share maps at rendezvous encounters represented by the colored bars.}
    \label{fig:prox_graph}
\end{figure}

==> sections/figures_tex/7-figure-ros.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=\textwidth]{figures/wireframe.png}
        \caption{Wireframe of Testing Area}
        \label{fig:gazebo_experiment}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
        \includegraphics[width=\textwidth]{figures/rviz.png}
        \caption{Rviz from Policy Components}
    \end{subfigure}
    \caption{Gazebo simulation environment we developed for deployment. (a) wireframe of the test environment constructed with height maps; (b) the rviz visualization of the Policy Components from fig.~\ref{fig:execution}.}
    \label{fig:gazebo}
\end{figure}

==> sections/notation.tex <==
\section{Notation}

\alysson{This is used to help me organize the notation}



==> sections/reward.tex <==

\begin{figure*}[t!]
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{Moscow}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{NY}
    \end{subfigure}
     \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{Dubai}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{Tokyo}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{Beijing}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{DC}
    \end{subfigure}
     \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{London}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{prk01}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{air01}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\columnwidth}
        \includegraphics[width=\textwidth]{figures/results/128_cons01.png}
        \caption{cons01}
    \end{subfigure}
    \caption{Reward analysis.}
    \label{fig:reward_range}
\end{figure*}

==> sections/tables_short.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{ clllllll }
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{Philly}} &
  \multicolumn{1}{c}{\centering{NY}} &
  \multicolumn{1}{c}{\centering{DC}} &
  \multicolumn{1}{c}{\centering{Tokyo}} &
  \multicolumn{1}{c}{\centering{Beijing}} & 
  \multicolumn{1}{c}{\centering{Dubai}} \\ \cline{1-7}
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${12686\pm 1319}$} &
  \multicolumn{1}{l|}{\small${6992\pm 648}$} &
  \multicolumn{1}{l|}{\small${11849\pm 301}$} &
  \multicolumn{1}{l|}{\small${10120\pm 719}$} &
  \multicolumn{1}{l|}{\small${11538\pm 1279}$} &
  \multicolumn{1}{l|}{\small${14643\pm 1273}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${11263\pm 1012}$} &
  \multicolumn{1}{l|}{\small${6060\pm 377}$} &
  \multicolumn{1}{l|}{\small${11540\pm 1277}$} &
  \multicolumn{1}{l|}{\small${9579\pm 856}$} &
  \multicolumn{1}{l|}{\small${11209\pm 1126}$} &
  \multicolumn{1}{l|}{\small${13813\pm 1621}$} \\ \cline{1-7}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${11387\pm 799}$} &
  \multicolumn{1}{l|}{\small${6398\pm 782}$} &
  \multicolumn{1}{l|}{\small${10889\pm 549}$} &
  \multicolumn{1}{l|}{\small${9326\pm 614}$} &
  \multicolumn{1}{l|}{\small${10341\pm 980}$} &
  \multicolumn{1}{l|}{\small${13167\pm 1888}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${7934\pm 339}$} &
  \multicolumn{1}{l|}{\small${4607\pm 108}$} &
  \multicolumn{1}{l|}{\small${8048\pm 188}$} &
  \multicolumn{1}{l|}{\small${7056\pm 205}$} &
  \multicolumn{1}{l|}{\small${7174\pm 309}$} &
  \multicolumn{1}{l|}{\small${8061\pm 249}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{7152\pm 90}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4436\pm 117}$} &
  \multicolumn{1}{l|}{\small$\mathbf{7181\pm 218}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6500\pm 399}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6459\pm 274}$} &
  \multicolumn{1}{l|}{\small$\mathbf{7700\pm 413}$} \\ \cline{1-7} 

\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{Moscow}} &
  \multicolumn{1}{c}{\centering{Berlin}} &
  \multicolumn{1}{c}{\centering{Lisbon}} &
  \multicolumn{1}{c}{\centering{London}} &
  \multicolumn{1}{c}{\centering{Paris}} & 
  \multicolumn{1}{c}{\centering{Rio}} \\ \cline{1-7}
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${14613\pm 1117}$} &
  \multicolumn{1}{l|}{\small${11973\pm 1153}$} &
  \multicolumn{1}{l|}{\small${9034\pm 602}$} &
  \multicolumn{1}{l|}{\small${11818\pm 1354}$} &
  \multicolumn{1}{l|}{\small${11399\pm 735}$} &
  \multicolumn{1}{l|}{\small${13871\pm 1213}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${13634\pm 1361}$} &
  \multicolumn{1}{l|}{\small${10798\pm 1005}$} &
  \multicolumn{1}{l|}{\small${8312\pm 696}$} &
  \multicolumn{1}{l|}{\small${11109\pm 821}$} &
  \multicolumn{1}{l|}{\small${10826\pm 829}$} &
  \multicolumn{1}{l|}{\small${12475\pm 1582}$} \\ \cline{1-7}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${12989\pm 830}$} &
  \multicolumn{1}{l|}{\small${11729\pm 684}$} &
  \multicolumn{1}{l|}{\small${8338\pm 512}$} &
  \multicolumn{1}{l|}{\small${10558\pm 827}$} &
  \multicolumn{1}{l|}{\small${10359\pm 706}$} &
  \multicolumn{1}{l|}{\small${11140\pm 481}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${8297\pm 183}$} &
  \multicolumn{1}{l|}{\small${7632\pm 204}$} &
  \multicolumn{1}{l|}{\small${5964\pm 193}$} &
  \multicolumn{1}{l|}{\small${7760\pm 345}$} &
  \multicolumn{1}{l|}{\small${7436\pm 130}$} &
  \multicolumn{1}{l}{\small${8073\pm 282}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{7870\pm 316}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6932\pm 117}$} &
  \multicolumn{1}{l|}{\small$\mathbf{5712\pm 141}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6996\pm 116}$} &
  \multicolumn{1}{l|}{\small$\mathbf{7084\pm 170}$} &
  \multicolumn{1}{l|}{\small$\mathbf{7460\pm 295}$} \\ \cline{1-7}   

\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{prk01}} &
  \multicolumn{1}{c}{\centering{prk02}} &
  \multicolumn{1}{c}{\centering{prk03}} &
  \multicolumn{1}{c}{\centering{prk04}} &
  \multicolumn{1}{c}{\centering{air01}} &
  \multicolumn{1}{c}{\centering{air02}} \\ \cline{1-7}
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${10078\pm 881}$} &
  \multicolumn{1}{l|}{\small${2980\pm 285}$} &
  \multicolumn{1}{l|}{\small${7967\pm 744}$} &
  \multicolumn{1}{l|}{\small${4378\pm 186}$} &
  \multicolumn{1}{l|}{\small${5005\pm 656}$} &
  \multicolumn{1}{l|}{\small${10053\pm 1740}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${9000\pm 1098}$} &
  \multicolumn{1}{l|}{\small${3016\pm 235}$} &
  \multicolumn{1}{l|}{\small${7398\pm 597}$} &
  \multicolumn{1}{l|}{\small${4245\pm 315}$} &
  \multicolumn{1}{l|}{\small${4582\pm 329}$} &
  \multicolumn{1}{l|}{\small${10270\pm 1784}$} \\ \cline{1-7}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${9172\pm 802}$} &
  \multicolumn{1}{l|}{\small${2886\pm 165}$} &
  \multicolumn{1}{l|}{\small${6778\pm 512}$} &
  \multicolumn{1}{l|}{\small${4189\pm 184}$} &
  \multicolumn{1}{l|}{\small${4634\pm 497}$} &
  \multicolumn{1}{l|}{\small${9039\pm 868}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${5833\pm 251}$} &
  \multicolumn{1}{l|}{\small${2242\pm 49}$} &
  \multicolumn{1}{l|}{\small${5054\pm 182}$} &
  \multicolumn{1}{l|}{\small${3517\pm 101}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4310\pm 294}$} &
  \multicolumn{1}{l|}{\small${6985\pm 286}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{5458\pm 222}$} &
  \multicolumn{1}{l|}{\small$\mathbf{2226\pm 63}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4895\pm 265}$} &
  \multicolumn{1}{l|}{\small$\mathbf{3389\pm 159}$} &
  \multicolumn{1}{l|}{\small${4436\pm 215}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6538\pm 378}$} \\ \cline{1-7} 

\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{air03}} &
  \multicolumn{1}{c}{\centering{air04}} &
  \multicolumn{1}{c}{\centering{cons01}} &
  \multicolumn{1}{c}{\centering{cons02}} &
  \multicolumn{1}{c}{\centering{cons03}} &
  \multicolumn{1}{c}{\centering{cons04}} \\ \cline{1-7}
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${6460\pm 547}$} &
  \multicolumn{1}{l|}{\small${6710\pm 718}$} &
  \multicolumn{1}{l|}{\small${10822\pm 1690}$} &
  \multicolumn{1}{l|}{\small${7003\pm 495}$} &
  \multicolumn{1}{l|}{\small${7186\pm 496}$} &
  \multicolumn{1}{l|}{\small${5366\pm 464}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${6306\pm 469}$} &
  \multicolumn{1}{l|}{\small${6120\pm 601}$} &
  \multicolumn{1}{l|}{\small${9262\pm 622}$} &
  \multicolumn{1}{l|}{\small${6379\pm 400}$} &
  \multicolumn{1}{l|}{\small${6379\pm 400}$} &
  \multicolumn{1}{l|}{\small${4992\pm 342}$} \\ \cline{1-7}
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${6230\pm 661}$} &
  \multicolumn{1}{l|}{\small${6283\pm 682}$} &
  \multicolumn{1}{l|}{\small${8764\pm 644}$} &
  \multicolumn{1}{l|}{\small${6451\pm 302}$} &
  \multicolumn{1}{l|}{\small${6388\pm 495}$} &
  \multicolumn{1}{l|}{\small${5094\pm 511}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${5197\pm 618}$} &
  \multicolumn{1}{l|}{\small${5427\pm 361}$} &
  \multicolumn{1}{l|}{\small${7034\pm 338}$} &
  \multicolumn{1}{l|}{\small${4954\pm 184}$} &
  \multicolumn{1}{l|}{\small$\mathbf{5343\pm 216}$} &
  \multicolumn{1}{l|}{\small${4237\pm 184}$} \\ \cline{1-7} 
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{5023\pm 416}$} &
  \multicolumn{1}{l|}{\small$\mathbf{5263\pm 307}$} &
  \multicolumn{1}{l|}{\small$\mathbf{6553\pm 293}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4717\pm 123}$} &
  \multicolumn{1}{l|}{\small${5449\pm 260}$} &
  \multicolumn{1}{l|}{\small$\mathbf{4064\pm 129}$} \\ \cline{1-7} 
\end{tabular}
}
\caption{Benchmark results for our dataset composed of cities, parking lots (prk), airport sections (air), and constructions sites (cons).}
\label{tab:table_cities}
\vspace{-2.0em}
\end{table*}


==> sections/tablesbkp.tex <==
\begin{table*}[t!]
\centering
\resizebox{1.2\textwidth}{!}{
\begin{tabular}{ clllllllllllll }
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{Philly}} &
  \multicolumn{1}{c}{\centering{NY}} &
  \multicolumn{1}{c}{\centering{DC}} &
  \multicolumn{1}{c}{\centering{Tokyo}} &
  \multicolumn{1}{c}{\centering{Beijing}} & 
  \multicolumn{1}{c}{\centering{Dubai}} &
  \multicolumn{1}{c}{\centering{Moscow}} &
  \multicolumn{1}{c}{\centering{Berlin}} &
  \multicolumn{1}{c}{\centering{Lisbon}} &
  \multicolumn{1}{c}{\centering{London}} &
  \multicolumn{1}{c}{\centering{Paris}} & 
  \multicolumn{1}{c}{\centering{Rio}} \\ \cline{1-13}
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${12686\pm 1319}$} & %Philly
  \multicolumn{1}{l|}{\small${6992\pm 648}$} & %NY
  \multicolumn{1}{l|}{\small${11849\pm 301}$} & %DC
  \multicolumn{1}{l|}{\small${10120\pm 719}$} & %Tokyo
  \multicolumn{1}{l|}{\small${11538\pm 1279}$} & %Beijing
  \multicolumn{1}{l|}{\small${14643\pm 1273}$} & %Dubai
  \multicolumn{1}{l|}{\small${14613\pm 1117}$} & %Moscow
  \multicolumn{1}{l|}{\small${11973\pm 1153}$} & %Berlin
  \multicolumn{1}{l|}{\small${9034\pm 602}$} & %Lisbon
  \multicolumn{1}{l|}{\small${11818\pm 1354}$} & %London
  \multicolumn{1}{l|}{\small${11399\pm 735}$} & %Paris
  \multicolumn{1}{l}{\small${13871\pm 1213}$} \\ \cline{1-13}  %Rio
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${11263\pm 1012}$} &  %Philly
  \multicolumn{1}{l|}{\small${6060\pm 377}$} & %NY
  \multicolumn{1}{l|}{\small${11540\pm 1277}$} &%DC
  \multicolumn{1}{l|}{\small${9579\pm 856}$} &%Tokyo
  \multicolumn{1}{l|}{\small${11209\pm 1126}$} &%Beijing
  \multicolumn{1}{l|}{\small${13813\pm 1621}$} &%Dubai
  \multicolumn{1}{l|}{\small${13634\pm 1361}$} & %Moscow
  \multicolumn{1}{l|}{\small${10798\pm 1005}$} &%Berlin
  \multicolumn{1}{l|}{\small${8312\pm 696}$} &%Lisbon
  \multicolumn{1}{l|}{\small${11109\pm 821}$} & %London
  \multicolumn{1}{l|}{\small${10826\pm 829}$} &%Paris
  \multicolumn{1}{l}{\small${12475\pm 1582}$} \\ \cline{1-13} %Rio
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${11387\pm 799}$} &%Philly
  \multicolumn{1}{l|}{\small${6398\pm 782}$} & %NY
  \multicolumn{1}{l|}{\small${10889\pm 549}$} &%DC
  \multicolumn{1}{l|}{\small${9326\pm 614}$} &%Tokyo
  \multicolumn{1}{l|}{\small${10341\pm 980}$} &%Beijing
  \multicolumn{1}{l|}{\small${13167\pm 1888}$} &%Dubai
  \multicolumn{1}{l|}{\small${12989\pm 830}$} & %Moscow
  \multicolumn{1}{l|}{\small${11729\pm 684}$} &%Berlin
  \multicolumn{1}{l|}{\small${8338\pm 512}$} &%Lisbon
  \multicolumn{1}{l|}{\small${10558\pm 827}$} &%London
  \multicolumn{1}{l|}{\small${10359\pm 706}$} &%Paris
  \multicolumn{1}{l}{\small${11140\pm 481}$} \\ \cline{1-13} %Rio
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${7934\pm 339}$} &%Philly
  \multicolumn{1}{l|}{\small${4607\pm 108}$} &%NY
  \multicolumn{1}{l|}{\small${8048\pm 188}$} &%DC
  \multicolumn{1}{l|}{\small${7056\pm 205}$} &%Tokyo
  \multicolumn{1}{l|}{\small${7174\pm 309}$} &%Beijing
  \multicolumn{1}{l|}{\small${8061\pm 249}$} &%Dubai
  \multicolumn{1}{l|}{\small${8297\pm 183}$} &%Moscow
  \multicolumn{1}{l|}{\small${7632\pm 204}$} &%Berlin
  \multicolumn{1}{l|}{\small${5964\pm 193}$} &%Lisbon
  \multicolumn{1}{l|}{\small${7760\pm 345}$} &%London
  \multicolumn{1}{l|}{\small${7436\pm 130}$} &%Paris
  \multicolumn{1}{l}{\small${8073\pm 282}$} \\ \cline{1-13} %Rio
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{7152\pm 90}$} &%Philly
  \multicolumn{1}{l|}{\small$\mathbf{4436\pm 117}$} &%NY
  \multicolumn{1}{l|}{\small$\mathbf{7181\pm 218}$} &%DC
  \multicolumn{1}{l|}{\small$\mathbf{6500\pm 399}$} &%Tokyo
  \multicolumn{1}{l|}{\small$\mathbf{6459\pm 274}$} &%Beijing
  \multicolumn{1}{l|}{\small$\mathbf{7700\pm 413}$} &%Dubai
  \multicolumn{1}{l|}{\small$\mathbf{7870\pm 316}$} &%Moscow
  \multicolumn{1}{l|}{\small$\mathbf{6932\pm 117}$} &%Berlin
  \multicolumn{1}{l|}{\small$\mathbf{5712\pm 141}$} &%Lisbon
  \multicolumn{1}{l|}{\small$\mathbf{6996\pm 116}$} &%London
  \multicolumn{1}{l|}{\small$\mathbf{7084\pm 170}$} &%Paris
  \multicolumn{1}{l}{\small$\mathbf{7460\pm 295}$} \\ \cline{1-13} %Rio
  
\multicolumn{1}{l}{} &
  \multicolumn{1}{c}{\centering{prk01}} &%prk01
  \multicolumn{1}{c}{\centering{prk02}} &%prk02
  \multicolumn{1}{c}{\centering{prk03}} &%prk03
  \multicolumn{1}{c}{\centering{prk04}} &%prk04
  \multicolumn{1}{c}{\centering{air01}} &%air01
  \multicolumn{1}{c}{\centering{air02}} &%air02
  \multicolumn{1}{c}{\centering{air03}} &%air03
  \multicolumn{1}{c}{\centering{air04}} &%air04
  \multicolumn{1}{c}{\centering{cons01}} &%cons01
  \multicolumn{1}{c}{\centering{cons02}} &%cons02
  \multicolumn{1}{c}{\centering{cons03}} &%cons03
  \multicolumn{1}{c}{\centering{cons04}} \\ \cline{1-13}%cons04
\multicolumn{1}{c|}{BS} &
  \multicolumn{1}{l|}{\small${10078\pm 881}$} &%prk01
  \multicolumn{1}{l|}{\small${2980\pm 285}$} &%prk02
  \multicolumn{1}{l|}{\small${7967\pm 744}$} &%prk03
  \multicolumn{1}{l|}{\small${4378\pm 186}$} &%prk04
  \multicolumn{1}{l|}{\small${5005\pm 656}$} &%air01
  \multicolumn{1}{l|}{\small${10053\pm 1740}$} &%air02
  \multicolumn{1}{l|}{\small${6460\pm 547}$} &%air03
  \multicolumn{1}{l|}{\small${6710\pm 718}$} &%air04
  \multicolumn{1}{l|}{\small${10822\pm 1690}$} &%cons01
  \multicolumn{1}{l|}{\small${7003\pm 495}$} &%cons02
  \multicolumn{1}{l|}{\small${7186\pm 496}$} &%cons03
  \multicolumn{1}{l}{\small${5366\pm 464}$} \\ \cline{1-13} %cons04
\multicolumn{1}{c|}{CRN1R} &
  \multicolumn{1}{l|}{\small${9000\pm 1098}$} &%prk01
  \multicolumn{1}{l|}{\small${3016\pm 235}$} &%prk02
  \multicolumn{1}{l|}{\small${7398\pm 597}$} &%prk03
  \multicolumn{1}{l|}{\small${4245\pm 315}$} &%prk04
  \multicolumn{1}{l|}{\small${4582\pm 329}$} &%air01
  \multicolumn{1}{l|}{\small${10270\pm 1784}$} &%air02
  \multicolumn{1}{l|}{\small${6306\pm 469}$} &%air03
  \multicolumn{1}{l|}{\small${6120\pm 601}$} &%air04
  \multicolumn{1}{l|}{\small${9262\pm 622}$} &%cons01
  \multicolumn{1}{l|}{\small${6379\pm 400}$} &%cons02
  \multicolumn{1}{l|}{\small${6379\pm 400}$} &%cons03
  \multicolumn{1}{l}{\small${4992\pm 342}$} \\ \cline{1-13}%cons04
\multicolumn{1}{c|}{CRN2R} &
  \multicolumn{1}{l|}{\small${9172\pm 802}$} &%prk01
  \multicolumn{1}{l|}{\small${2886\pm 165}$} &%prk02
  \multicolumn{1}{l|}{\small${6778\pm 512}$} &%prk03
  \multicolumn{1}{l|}{\small${4189\pm 184}$} &%prk04
  \multicolumn{1}{l|}{\small${4634\pm 497}$} &%air01
  \multicolumn{1}{l|}{\small${9039\pm 868}$} &%air02
  \multicolumn{1}{l|}{\small${6230\pm 661}$} &%air03
  \multicolumn{1}{l|}{\small${6283\pm 682}$} &%air04
  \multicolumn{1}{l|}{\small${8764\pm 644}$} &%cons01
  \multicolumn{1}{l|}{\small${6451\pm 302}$} &%cons02
  \multicolumn{1}{l|}{\small${6388\pm 495}$} &%cons03
  \multicolumn{1}{l}{\small${5094\pm 511}$} \\ \cline{1-13} %cons04
\multicolumn{1}{c|}{Ours} &
  \multicolumn{1}{l|}{\small${5833\pm 251}$} &%prk01
  \multicolumn{1}{l|}{\small${2242\pm 49}$} &%prk02
  \multicolumn{1}{l|}{\small${5054\pm 182}$} &%prk03
  \multicolumn{1}{l|}{\small${3517\pm 101}$} &%prk04
  \multicolumn{1}{l|}{\small$\mathbf{4310\pm 294}$} &%air01
  \multicolumn{1}{l|}{\small${6985\pm 286}$} &%air02
  \multicolumn{1}{l|}{\small${5197\pm 618}$} &%air03
  \multicolumn{1}{l|}{\small${5427\pm 361}$} &%air04
  \multicolumn{1}{l|}{\small${7034\pm 338}$} &%cons01
  \multicolumn{1}{l|}{\small${4954\pm 184}$} &%cons02
  \multicolumn{1}{l|}{\small$\mathbf{5343\pm 216}$} &%cons03
  \multicolumn{1}{l}{\small${4237\pm 184}$} \\ \cline{1-13} %cons04
\multicolumn{1}{c|}{OursSync} &
  \multicolumn{1}{l|}{\small$\mathbf{5458\pm 222}$} &%prk01
  \multicolumn{1}{l|}{\small$\mathbf{2226\pm 63}$} &%prk02
  \multicolumn{1}{l|}{\small$\mathbf{4895\pm 265}$} &%prk03
  \multicolumn{1}{l|}{\small$\mathbf{3389\pm 159}$} &%prk04
  \multicolumn{1}{l|}{\small${4436\pm 215}$} &%air01
  \multicolumn{1}{l|}{\small$\mathbf{6538\pm 378}$} &%air02
  \multicolumn{1}{l|}{\small$\mathbf{5023\pm 416}$} &%air03
  \multicolumn{1}{l|}{\small$\mathbf{5263\pm 307}$} &%air04
  \multicolumn{1}{l|}{\small$\mathbf{6553\pm 293}$} &%cons01
  \multicolumn{1}{l|}{\small$\mathbf{4717\pm 123}$} &%cons02
  \multicolumn{1}{l|}{\small${5449\pm 260}$} &%cons03
  \multicolumn{1}{l}{\small$\mathbf{4064\pm 129}$} \\ \cline{1-13} %cons04
\end{tabular}
}
\caption{Benchmark results for our dataset composed of cities, parking lots (prk), airport sections (air), and constructions sites (cons). }
\label{tab:table_cities}
\vspace{-2.0em}
\end{table*}

